Navigation with QPHIL: Quantizing Planner for Hierarchical Implicit Q-Learning

Offline Reinforcement Learning (RL) has emerged as a powerful alternative to imitation learning for behavior modeling in various domains, particularly in complex navigation tasks. An existing challenge with Offline RL is the signal-to-noise ratio, i.e. how to mitigate incorrect policy updates due to errors in value estimates. Towards this, multiple works have demonstrated the advantage of hierarchical offline RL methods, which decouples high-level path planning from low-level path following. In this work, we present a novel hierarchical transformer-based approach leveraging a learned quantizer of the space. This quantization enables the training of a simpler zone-conditioned low-level policy and simplifies planning, which is reduced to discrete autoregressive prediction. Among other benefits, zone-level reasoning in planning enables explicit trajectory stitching rather than implicit stitching based on noisy value function estimates. By combining this transformer-based planner with recent advancements in offline RL, our proposed approach achieves state-of-the-art results in complex long-distance navigation environments.

==> __additional_related.tex <==
\section{Additional related work}

\textbf{Algorithms that may be useful for benchmarks:}


GCBC: Learning to Reach Goals via
Iterated Supervised Learning

WGCBC: RETHINKING GOAL-CONDITIONED SUPERVISED
LEARNING AND ITS CONNECTION TO OFFLINE RL \cite{yang2022rethinking}

GC-IQL: OFFLINE REINFORCEMENT LEARNING
WITH IMPLICIT Q-LEARNING

GC-POR: A Policy-Guided Imitation Approach for
Offline Reinforcement Learning

HGCBC: Relay Policy Learning: Solving Long-Horizon Tasks
via Imitation and Reinforcement Learning \cite{gupta2019relay}

TAP: Published as a conference paper at ICLR 2023
EFFICIENT PLANNING IN A COMPACT LATENT ACTION
SPACE

WT: Waypoint Transformer: Reinforcement Learning via
Supervised Learning with Intermediate Targets

HDMI: (diffusion + hierarchical planning)\cite{pmlr-v202-li23ad} 

VQ-VAE: Neural Discrete Representation Learning

HIPS: Hierarchical Imitation Learning with Vector Quantized Models

\textbf{Hierachical (Online) Goal Conditioned RL}: 


Goal-conditioned reinforcement learning with imagined subgoals (2021): Au cours du training, on génère des subgoals sg pour aller de s à g via une politque high level, qui permet de guider l'apprentissage de la politique low level qui s'appuie sur l'action ag de s à sg pour aller de s à g, en online off-policy RL.


Feudal Reinforcement Learning(1992): Vieux papier pour la légacy, mais même idée générale.\cite{dayan1992feudal}


Hierarchical deep reinforcement learning (2016): Integrating temporal abstraction and intrinsic motivation: Version hierarchique du DQN pour le goal conditioned RL. \cite{kulkarni2016hierarchical}


Learning Multi-Level Hierarchies with Hindsight (2017):  Propose une approche hierarchique au goal conditioned RL online par le training en parallèle de k-politiques stackées, avec hindsight experience replay. \cite{levy2017learning}







==> __notes_pour_related.tex <==
\section{Notes to redact the related work}

In \cite{tan2021vimpac} they learn masked token prediction on discretized videos where tokens are generated using a vq-vae. They also use a contrastive loss but on the transformer, not the tokenization.\\

An exemple of VQ-VAE tokenization that goes to sequence prediction~\cite{lee2024leveraging}.\\

In \cite{9826807} they proposed a hierachical method that combine a low-level offline RL one and a high level planner. The high level model is a VAE and uses the value function of the low level policy to make the planning.\\

we build upon prior work and apply contrastive representation learning to action-labeled trajectories, in such a way that the (inner product of) learned representations exactly corresponds to a goal-conditioned value function \cite{eysenbach2022contrastive}.\\

In \cite{parisotto2020stabilizing} they say that transformers are difficult to optimize for especially in RL and propose to improve stability and learning speed.\\

\cite{chiappa2017recurrent} recurrent model that can make temporally and spatially coherent predictions for hundreds of time-steps into the future\\

\cite{bakker2001reinforcement} RL using LSTM in 2001. Nothing much but yeah\\

\cite{sermanet2018time, nair2022r3m, ma2022vip} employ the same l2 parameterization as HILPs to obtain temporal distance-based representations.\\

\cite{yamagata2023q} DT cannot stich. And it is worse what the dataset only contains suboptimal trajectories. So they propose QDT. ``It utilises the Dynamic Programming results to relabel the return-to-go in the training data to then train the DT with the relabelled data.''\\

\cite{ma2024rethinking} `` At the time of making decisions, a *high-level* policy first proposes an ideal *prompt* for the current state, a *low-level* policy subsequently generates an action conditioned on the given prompt. We show DT emerges as a special case of this framework with certain choices of high-level and low-level policies, and discuss the potential failure of these choices. Inspired by these observations, we study how to jointly optimize the high-level and low-level policies to enable the stitching ability, which further leads to the development of new offline RL algorithms. Our empirical results clearly show that the proposed algorithms significantly surpass DT on several control and navigation benchmarks. We hope our contributions can inspire the integration of transformer architectures within the field of RL.''

Trajectory Autoencoding Planner (TAP), which learns low-dimensional latent action codes with a state-conditional VQ-VAE.\cite{jiang2022efficient}\\

\cite{czechowski2021subgoal} Hierachical RL. They generate subgoals \(k\)-step ahead using a transformer module coupled with best first search.\\

\cite{jurgenson2020sub} plan subgoals suing the following: they plan an intermediate goal between the current state and the final goal and the recursively plan subgoals at the center of each new segment.\\

\cite{sudhakaran2023skill} skill decision transformer. They discover ``skills'' using a simple VQVAE and then have a transformer that predict action from latents. They are different than us because they do not use a contrastive loss and both are trained at the same time. Furthermore they do not plan subgoals. (Its just a workshop paper and they bad. But they are close enough that it would be weird not talking about them)\\

\cite{allshire2021laser} they learn a latent action space because most of times, the whole action space is not suitable. Then they learn a policy on this latent action space.\\

\cite{jiang2019language} ``Our approach learns an instruction-following low-level policy and a high-level policy that can reuse abstractions across tasks, in essence, permitting agents to reason using structured language.''\\

\cite{zawalski2022fast} ``AdaSubS generates diverse sets of subgoals at different distances. A verification mechanism is employed to filter out unreachable subgoals swiftly, allowing to focus on feasible further subgoals''\\

\cite{chen2021decision} ``By conditioning an autoregressive model on the desired return (reward), past states, and actions, our Decision Transformer model can generate future actions that achieve the desired return.''\\

\cite{kang2024efficient} random diffusion and they can combine with other methods such as IQL and improve on them. From my understanding, it is not hierarchic, they just use the loss from other methods. But I need to explore more.\\

HIQL \cite{park2024hiql}\\

\cite{kim2021landmark} (HIGL) they generate landmarks (important state) from traces and use that to construct a graph. Next landmark is chosen as the first landmark to explore using a shortest-path to the goal in the graph. A high level policy is trained to generate subgoals that are reachable and toward the landmark.\\
Landmark-Guided Subgoal Generation in Hierarchical Reinforcement Learning (2021): Two landmark selection schemes, one for coverage and one for exploration, alternating.

\cite{hausman2017multi} ``propose a multi-modal imitation learning framework that is able to segment and imitate skills from unlabelled and un- structured demonstrations by learning skill segmentation and imitation learning jointly.'' (they use GANs)\\


IQL \cite{kostrikov2021offline}\\

GCBC \cite{emmons2021rvs}\\

D3IL \cite{jia2024towards}\\

Waypoint transformer \cite{badrinath2024waypoint} A model is trained to predict the state \(k\) step further. A trasnformer is used as a policy. It is conditionned by previous states and waypoints.\\

\cite{kujanpaa2024hybrid} planning with compleness guarenties. They sue a two fold hierachical methode.

HIPS \cite{kujanpaa2023hierarchical} They find generate waypoints suing RL: they train a detector (it give probability to each state in the H following states during training) and the reward is based how well a co-trained REINFORCE is able to predict the next action when given the waypoint instead of the goal (and there is a penalty to avoid using too much waypoints). This gives them a dataset of subgoal pairs. Then they use a VQ-VAE trained on this dataset to generate waypoints.\\

Trajectory Transformer \cite{janner2021offline}. The discretise state and action. Each dimension is discretized independently. In goal conditionned offline RL, they use a IQL-like Q-function to performe a beam search.\\

VQ-BeT \cite{lee2024behavior} tokenize continuous actions with a hierarchical vector quantization module. Main difference is the the actions are tokenized instead of states and that they do not use contrastive loss for tokenization. They have a mini-GPT network that has two heads. One select a token and the other one is an offset to had to the token. This way, they have continuous actions.\\

\cite{gao2023adaptive} really vision centered. They segment space into zones and navigate from zone to zone to reach the goal. 


\cite{eysenbach2019search} Search on the Replay Buffer: Bridging Planning and Reinforcement Learning (2019): Builds a path finding graph from a collected experience replay buffer to perform pathfinding for high level policy. Distances or computed by value estimation using DQN and DDPG. Then, use low level policy to navigation.

\cite{hoang2021successor} Successor Feature Landmarks for Long-Horizon Goal-Conditioned Reinforcement Learning (2021): Use Successor features to find temporal similarity betwwen states. Builds a planing graph with it. Also gives a way to solve perceptual aliasing in Doom.

\cite{huang2019mapping} Mapping State Space using Landmarks for Universal Goal Reaching (2019): Uses farthest point sampling to select landmark states to build a graph and perform path finding.

\cite{kim2023imitating} IMITATING GRAPH-BASED PLANNING WITH GOAL-CONDITIONED POLICIES (2023): Uses self imitation learning in hierachical way to transfers knowledge from a planner along with a graph into policy learning. They combine HER with subgoal skipping to improve performance.

\cite{nasiriany2019planning} Planning with Goal-Conditioned Policies (2019): Uses VAEs to encode subgoals like images as latent vectors, which is easier to generate as subgoals.

\cite{savinov2018semi} SEMI-PARAMETRIC TOPOLOGICAL MEMORY FOR NAVIGATION (2018): They use a similarity network trained by contrastive loss, if two observations are temporally near or not. To localize, they take a temporal window, and take the major (or discounted weighted locations). They build a graph, perform path finding with Dijkstra, and have a locomotion policy.

\cite{zhang2021world} World Model as a Graph: Learning Latent Landmarks for Planning (2021): First, how can we group together goals that are easily reachable from one another? The answer is to embed goals into a latent space, where the latent representation captures some notion of temporal distance between goals – in the sense that goals that would take many timesteps to navigate between are further apart in latent space. Second, we need to find a way to learn a sparse set of landmarks used for planning. Our method performs clustering on the constrained latent space, and decodes the learned centroids as the landmarks we seek. Finally, we need to develop a non-parametric planning algorithm responsible for selecting sequences of landmarks the agent must traverse to accomplish its high-level goal. They use graphs in the latent space of goals. They want to do clusters, they don't use VQ-VAE, but continuous VAEs with the Greedy Latent Sparsification. They use the Floyd algorithm for planing.

\cite{zhang2020generating} Generating adjacency-constrained subgoals in hierarchical reinforcement learning (2021): Helps high level policy training by restricting high level action space.

\cite{vezhnevets2017feudal} Feudal networks for hierarchical reinforcement learning (2017): Hierarchical policies en RNN, qui partagent une représentation commune apprise des états.

\cite{schmidhuber1991learning} Learning to generate sub-goals for action sequences (1991): Vieux papier legacy qui parle de hierarchical. 

Near-optimal representation learning for hierarchical reinforcement learning (2019): Ce papier aborde la question de la représentation des subgoals pour la polituique low level. Il comparent différentes manières de réprésenter les subgoals, de manière à aider l'apprentissage (raw x,y vs images vs latents etc.) et calculent une borne d'optimalité pour leur représentations. \cite{nachum2018near}

Data-efficient hierarchical reinforcement learning (2018): Propose une approche hierarchique au RL, avec une lower et une higher, qui optimizent des rewards hierarchiques.\cite{nachum2018data}




==> figures/tokenization_exemple.tex <==
\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{.45\textwidth}
        \includegraphics[width=\textwidth]{figures/godot}
        \caption{An in-house game}
        \label{fig:godot_tokenization_exemple}
    \end{subfigure}
    \begin{subfigure}[b]{.45\textwidth}
        \includegraphics[width=\textwidth]{figures/background_tokens_utra.pickle}
        \caption{Antmaze Ultra}
        \label{fig:tokenization-exemple_tokenization_exemple}
    \end{subfigure}
    \caption{Tokenization example. Each token has an associated color. The color of each point in the background correspond to the color of the associated token. It is noticeable that the tokens align with the walls thanks to the contrastive loss.}
\end{figure}

==> sections/HIQL_mathieu.tex <==
\paragraph*{Implicit Q-Learning (IQL)}
The main issue of offline RL is the overestimation of the value of out-of-distribution actions when minimizing the temporal difference error leading the policy to favor overestimated actions:
\begin{equation}
    \label{td_loss}
    \mathcal{L}_{TD} = \mathbb{E}_{(s_t,a_t,s_{t+1}) \sim \mathcal{D}} \left [  (r(s_t,a_t) + \gamma \; \underset{a_{t+1}}{\max} \; Q_{\hat{\theta}_Q}(s_{t+1},a_{t+1})-Q_{\theta_Q}(s_t,a_t))^2 \right ]
\end{equation}
with \(r(s_t,a_t)\) the task reward, \(\hat{\theta}_Q\) the parameters of a target network. Without further interactions with the environment, those overestimations cannot be corrected. While other work propose to regularize the loss function to avoid sampling out-of-distribution actions, \cite{kostrikov2021offline} proposes IQL which estimates the in-distribtion \(\max Q\) operator with expectile regression. To do so, it learns a state value function \(V_{{\theta}_V}(s_t)\) along a state-action value function \(Q_{{\theta}_{Q}}(s_t,a_t)\):
\begin{align}
    \label{iql_losses}
    \mathcal{L}_V(\theta_V) & = \mathbb{E}_{(s_t,a_t) \sim \mathcal{D}} \left [ L_2^\tau(Q_{\hat{\theta}_Q}(s_t,a_t) - V_{\theta_V}(s_t)) \right ] \\
    \mathcal{L}_Q(\theta_Q) & = \mathbb{E}_{(s_t,a_t,s_{t+1}) \sim \mathcal{D}} [ r(s_t,a_t) + \gamma \; V_{\theta_V}(s_{t+1})-Q_{\theta_Q}(s_t,a_t))^2 ]
\end{align}
with \(L_2^\tau(u) = |\tau - \mathbbm{1}(u < 0)|u^2, \tau \in [0.5,1)\) the expectile loss, which corresponds to an asymmetric square loss which penalises positive values more than negative ones the more \(\tau\) tends to \(1\), consequently leading \(V_{\theta_V}(s_t)\) to lean towards \( \max_{\; a_{t+1} \in \mathcal{A}, \text{ st. } \pi_\beta(a_{t}|s_t) > 0} \; Q_{\hat{\theta}_Q}(s_t,a_t)\) with \(\pi_\beta\) the datasets behavior policy.
The use of two different networks is justified to train the value function only on the dataset action distribution without incorporating environment dynamics in the TD-error loss, which avoids the overestimation induced by lucky transitions. Then, the trained \(V_{{\theta}_V}(s_t)\) and \(Q_{{\theta}_{Q}}(s_t,a_t)\) are used to compute advantages to extract a policy \(\pi_{\theta_\pi}\) with advantage weighted regression (AWR):
\begin{equation}
\label{awr_loss}
    \mathcal L_\pi(\theta_\pi) = -\mathbb E_{(s_t,a_t) \sim \mathcal D} \left[ \exp\left(\beta(Q_{\hat{\theta}_Q}(s_t,a_t) - V_{\theta_V}(s_t)\right)\log \pi_{\theta_\pi}(a_t|s_t) \right],
\end{equation}
with  \(\beta \in (0, +\infty]\) an inverse temperature. This correspond to the cloning of the demonstrations with a biais towards actions that present a higher Q-value.

\paragraph*{Hierarchical Implicit Q-Learning (HIQL)}
In the offline GCRL setting, the rewards are sparse, only giving signals for states where the goal is reached. Hence, as bad actions can be corrected by good actions and good actions can be polluted by bad actions in the future of the trajectory, offline RL methods are at risk of wrongly label bad actions as good one, and conversely good actions as bad ones. This leads to the learning of a noisy goal-condidtioned value function: \(\hat{V}(s_t,g) = V^*(s_t,g) + N(s_t,g)\) where \(V^*\) corresponds to the optimal value function and \(N\) corresponds to a noise. As the 'signal-to-noise' ratio worsens for longer term goals, offline RL methods such as IQL struggle when the scale of the GCRL problem increases, leading to noisy advantages in IQL's AWR weights for which the noise overtakes the signal. To alleviate this issue, HIQL proposes to learn a noisy goal conditioned action-free value function as in IQL: 
\begin{equation}
    \label{iqlv}
    \mathcal{L}_V(\theta_V) = \mathbb{E}_{(s_t,s_{t+1}) \sim \mathcal{D}, g \sim p(g|\tau)} \left [ L_2^\tau(r(s_t,g) + \gamma V_{\hat{\theta}_V}(s_{t+1},g) - V_{\theta_V}(s_t,g)) \right ]
\end{equation}
and to use it to learn two policies \(\pi^h(s_{t+k}|s_t,g)\) to generate subgoals from the goal and \(\pi^l(a_t|s_t,g)\) to generate actions to reach the subgoals:
\begin{align}
    \label{iql_losses}
    \mathcal{L}_{\pi^h}(\theta_h) & = \mathbb{E}_{(s_t,s_{t+k},g)}[\exp (\beta \cdot (V_{\theta_V}(s_{t+k},g) - V_{\theta_V}(s_t,g))) \log \pi_{\theta_h}^h(s_{t+k}|s_t,g)] \\
    \mathcal{L}_{\pi^l}(\theta_l) & = \mathbb{E}_{(s_t,a_t,s_{t+1},s_{t+k})}[\exp(\beta \cdot (V_{\theta_V}(s_{t+1},s_{t+k}) - V_{\theta_V}(s_t,s_{t+k})) \log \pi_{\theta_l}^l(a_t|s_t,s_{t+k})]
\end{align}
With this division, each policy profits from higher signal-to-noise ratios as the low-policy only queries the value function for nearby subgoals \(V(s_{t+1},s_{t+k})\) and the high policy queries the value function for more diverse states leading to dissimilar values \(V(s_{t+k},g)\).

==> sections/mathieu_additions.tex <==
\subsection{Theorical interpretation and motivation (Proposition d'explication sur pourquoi on bat HIQL, à travailler)}


\section{Can replanning improve the navigation performance of QPHIL ?}
QPHIL high policy can allow full planning in an open-loop manner. We plan the sequence of subgoals at the start the the episode and don't perform any further replanning. The the tokens are depiled forever once they are been reached. However, if the low policy makes a mistake and goes into another token, which we call "lost", it might get into out-of-distribution \(\pi(a|s,i)\) where \(s\) is now too far from \(i\) (not in a neighbour area). In the following, we analyze the effect of several replaning on the performance and the inference time of our agent.

\begin{itemize}
    \item \textbf{Go-back replaning:}  This replaning replans when a out-of-path token is detected. It consists in putting back the former current token on the top of the subgoal pile in order to go back to it.
    \item \textbf{Full-replaning:} This replaning replans when a out-of-path token is detected. The whole path, considering the new token as the new starting token, is replanned.
    \item \textbf{n-step replaning:} This replaning replans every n timesteps. The whole path, considering the new token as the new starting token, is replanned.
\end{itemize}

\subsection{Results}
On antmaze-extreme-diverse:
\begin{table}[H]
    \caption{Results on antmaze environments. Italique=sans grid search. Vert=meilleur que HIQL}
    \centering
    \scriptsize
    % \renewcommand{\arraystretch}{.8}
    \begin{tabularx}{\textwidth}{ccccCCccccc}
    \Xhline{.8pt}
    % \rowcolor{gray!20}
        Dataset & No replaning & go back & replan & 50-step\\
        \Xhline{.1pt}
        \makecell{success-rate} & 44.3 \std{14} & 35.6 \std{12.5} & 43.3 \std{13} & 1.0 \std{1.5}\\
        \makecell{success-rate-subgoal} & 45.5 \std{13.8} & 35.6 \std{12.5} & 44.3 \std{12.8} &  1.0 \std{1.5} \\
        \Xhline{.1pt}
        \makecell{n-inference} &  & & & \\
        \makecell{n-planning} & & & & \\
        \Xhline{.1pt}
        \makecell{n-ratio} &  & & & \\
        \makecell{planning-time} & & & &  \\
        \Xhline{.1pt}
        \makecell{inference-time} &  & &  & \\
        \makecell{time-proportion} & & & & \\
    \Xhline{.8pt}
        
        
    \end{tabularx}
    \label{fig:state-results}
\end{table}

\subsubsection{The importance of history vs memory free replaning}
We analyse here for each previous replaning the imporance  of having the history of the past sequence in the planning vs considering the current token as the new starting token.

\subsection{Impact of using argmax to not go back and forth}
When using n-step replaning, its important to not do back and forth of tokens, that's why you need to use argmax.
Our method right now only planned its trajectory one time at the beginning, and the tokens are depiled forever once they are reached. Such planning is very effective in term of compute ressource and enough if the low policy is performing its following well. However, if the low policy makes a mistake and goes into another token, which we call "lost", it might get into out-of-distribution \(\pi(a|s,i)\) where \(s\) is now too far from \(i\) (not in a neighbour area). We test several replaning methods in terms of: their impact on success rate, the number of planning steps that occured, and the pourcentage of inference time used for each.

\subsection{Possible narratif (à vérifier avec des maths)}
On veut faire du offline rl. En offline rl, il existe un important problème du singal-to-noise ratio. Ceci correspond au fait que l'action démontrée eb un état n'est que rarement la meilleur dans l'obtention d'un goal futur dans la trajectoire. Ainsi, on veut faire du RL, mais cependant, l'équation de Bellman peut présenter des rewards bruités, étant donné qu'une action a toujours un reward nul, donc aucun signal, sauf à l'atteinte du goal. Ainsi, c'est seulement en faisant remonter les signaux pour l'équation de Bellman que la Q function est apprise, mais celle-ci à une action donnée peut être élevée sans que cette action ne soit vraiment optimale. Ainsi, plus les trajectoires sont grandes en taille, moins les actions n'ont d'impact dans l'atteinte rapide (rewards à -1 sauf 0 à l'atteitne du goal) et efficiace du goal. Ainsi, on apprend une fonction valeur potentiellement bruitée aussi. Les méthodes hiérachiques telles que HIQL visent à réduire l'importance de ce problème en ajoutant un niveau hierarchique à la politique. Cependant, HIQL semble réduire le problème mais est quand même très concerné car sa fonction de valeur high level subit quand même ce genre de problèmes malgrès tout, et donc elle va générer des subgoals potentiellement sous optimaux. Aussi, ces subgoals doivent être générés par un modèle telle des actions, ce qui peut donner du fil à retordre à la low policy qui doit viser un subgoal puis potientiellement un autre en zig zag. Notre méthode vise à résoudre ce problème d'une différente manière en utilisant une politique hierarchique mais en changeant le paradigme high level, en utilisant de la quantization. Celle-ci peut à la fois résoudre les problème de bruit dans le  choix du subgoal suivant et elle donne à la low policy une information plus stable, ce qui lui permet d'augmenter en performance. A vérifier mathématiquement sur des exemples.


\subsection{Godot offline rl experiments}
TODO: Présenter l'envionnement Godot et les résultats dans le tableau d'expérience de Godot en success rate

Les résultats préliminaires sur godot sont: 
\begin{table}[H]
    \caption{Results on antmaze environments. Italique=sans grid search. Vert=meilleur que HIQL}
    \centering
    \scriptsize
    % \renewcommand{\arraystretch}{.8}
    \begin{tabularx}{\textwidth}{cccccccccc}
    \Xhline{.8pt}
    % \rowcolor{gray!20}
        Dataset & GCBC & GC-IQL & HGCBC & \makecell{HIQL\\ w/o\\ repr.} & \makecell{QGCBC\\ w/\\ aug.} & & \makecell{QGCBC\\ w/o\\ aug.} & \makecell{QPHIL\\ w/\\ aug.} & \makecell{QPHIL\\ w/o\\ aug.}\\
        \Xhline{.1pt}
        \makecell{godot} & 61.8\std{3.5} & 49.0\std{2.6} & 69.3\std{3.9} & 61.1\std{5.1} & & &  & \\
        \makecell{godot-raycast} & 78.6\std{2.3} & 76.8\std{2.8} & 95.1\std{2.2} & 91.8\std{2.3} &  & & &\\
        \Xhline{.1pt}
        
        
    \end{tabularx}
    \label{fig:state-results}
\end{table}
Ces résultats sont étonnants: imitation learning et offline rl semble plus ou moins forts, le hierarchique semble plus ou moins fort que le flat. Seul la présence de raycasts aide clairement. Dans l'attente d'une validation de ces résultats, et ayant besoin de GCBC et IQL, je ne lance pas de suite QPHIL.

\subsection{What about HIQL with BC in the high level policy \( high beta=0 \)}
I ran experiments on HIQL for antmaze-ultra-diverse-v0 with a high-beta = 0 on 8 seeds and I get: \(19.0 \pm 7.8\) mean success rate, so it is not improving. The point is that: the subgoal is a generated one, so like an action, there are good and bad subgoals in the dataset, if you don't do offline rl, you are screwed. So our gain is not about BC in high policy. It might be about lower signal to noise for high level (tokens), and low level: no high freq varying subgoals.

I reran those experiments but with high-beta = 0 and high-p-randomgoal=0. This time, we get the same perf has standard hiql, which doesn't go beyond the performance of our method.

\begin{table}[H]
    \caption{Results on antmaze environments. Italique=sans grid search. Vert=meilleur que HIQL}
    \centering
    \scriptsize
    \begin{tabularx}{\textwidth}{ccc}
    \Xhline{.8pt}
        Dataset & \makecell{BC+IQL\\ w/\\ repr.} & \makecell{BC+IQL\\ w/o\\ repr.} \\
        \Xhline{.1pt}
        \makecell{r-medium\\ play} & & \\
        \makecell{r-medium\\ diverse} & & \\
        \Xhline{.1pt}
        \makecell{r-large\\ play} & & \\
        \makecell{r-large\\ diverse} & & \\
        \Xhline{.1pt}
        \makecell{r-ultra\\ play} & 47.4 \std{15} & 43.2 \std{19} \\
        \makecell{r-ultra\\ diverse} & 50.8 \std{11}& 51.4 \std{17} \\
        \Xhline{.1pt}
        \makecell{r-extreme\\ play} & & \\
        \makecell{r-extreme\\ diverse} & & \\
    \Xhline{.8pt}
    \end{tabularx}
    \label{fig:state-results}
\end{table}

\subsection{Replanning}
Our method right now only planned its trajectory one time at the beginning, and the tokens are depiled forever once they are reached. Such planning is very effective in term of compute ressource and enough if the low policy is performing its following well. However, if the low policy makes a mistake and goes into another token, which we call "lost", it might get into out-of-distribution \(\pi(a|s,i)\) where \(s\) is now too far from \(i\) (not in a neighbour area). We test several replaning methods in terms of: their impact on success rate, the number of planning steps that occured, and the pourcentage of inference time used for each.

\subsubsection{Go-back replaning}
This replaning strategy consists in putting back the former current token on the top of the subgoal pile in order to go back to it.

\subsubsection{Replan replaning}
This replaning replans the all trajectory, considering the new token as the new starting token.

\subsubsection{n-step replaning}
This replaning replans every n-timesteps of the environment.

\subsubsection{Results}
On antmaze-extreme-diverse:
\begin{table}[H]
    \caption{Results on antmaze environments. Italique=sans grid search. Vert=meilleur que HIQL}
    \centering
    \scriptsize
    % \renewcommand{\arraystretch}{.8}
    \begin{tabularx}{\textwidth}{ccccCCccccc}
    \Xhline{.8pt}
    % \rowcolor{gray!20}
        Dataset & No replaning & go back & replan & 50-step\\
        \Xhline{.1pt}
        \makecell{success-rate} & 44.3 \std{14} & 35.6 \std{12.5} & 43.3 \std{13} & 1.0 \std{1.5}\\
        \makecell{success-rate-subgoal} & 45.5 \std{13.8} & 35.6 \std{12.5} & 44.3 \std{12.8} &  1.0 \std{1.5} \\
        \Xhline{.1pt}
        \makecell{n-inference} &  & & & \\
        \makecell{n-planning} & & & & \\
        \Xhline{.1pt}
        \makecell{n-ratio} &  & & & \\
        \makecell{planning-time} & & & &  \\
        \Xhline{.1pt}
        \makecell{inference-time} &  & &  & \\
        \makecell{time-proportion} & & & & \\
    \Xhline{.8pt}
        
        
    \end{tabularx}
    \label{fig:state-results}
\end{table}

\subsubsection{The importance of history vs memory free replaning}
We analyse here for each previous replaning the imporance  of having the history of the past sequence in the planning vs considering the current token as the new starting token.

\subsubsection{Impact of using argmax to not go back and forth}
When using n-step replaning, its important to not do back and forth of tokens, that's why you need to use argmax.

\subsection{Références}
[ 22 , 38 , 40, 45, 46 , 69, 78, 101 ] de HIQL.
\subsection{Impact of stithcing}
Comment est-ce que le stitching peut fonctioner if on en voit jamais vraiment tout la trajectoires, surement de proche en proche, ce qu'il faut vérifier. Ceci peut justifier l'utilisation d'un transofmrer et de son attention pour faire du stithcing implicite avec son attention, ce qui serait le remplacant d'une high policy $\pi(token_{k+1}|token_k,token_g)$.

% \begin{figure}[H]
%     \centering
%     \begin{tikzpicture}
%     \begin{axis}[
%         height=.25\textwidth,
%         width=.5\textwidth,
%         xticklabels=\empty=\empty,
%         % xlabel={Token index},
%         ylabel={Distance},
%         ybar,
%         bar width=1.,
%         xmax=97,
%         ymax=205
%     ]

%      \addplot+[
%         ybar,
%         fill=magenta!40!white,
%         draw=purple,
%         bar shift=1
%         % opacity=.5
%     ] table [x index=0, y index=1] {data/max_non_constrastive_distances.txt}; 
%     \addplot+[
%         ybar,
%         fill=cyan!40!white,
%         draw=blue,
%         bar shift=.9
%         % opacity=.4
%     ] table [x index = 0, y index=1] {data/min_non_constrastive_distances.txt};

%     \end{axis}
%     \end{tikzpicture}\\ \vspace{-.3cm}
%     \begin{tikzpicture}
%     \begin{axis}[
%         height=.25\textwidth,
%         width=.5\textwidth,
%         xlabel={Token index},
%         ylabel={Distance},
%         ybar,
%         bar width=1.,
%         xmax=97,
%         ymax=205
%     ]

%      \addplot[
%         ybar,
%         fill=magenta!40!white,
%         draw=purple,
%         bar shift=1
%         % opacity=.5
%     ] table [x index=0, y index=1] {data/max_constrastive_distances.txt}; 
%     \addplot[
%         ybar,
%         fill=cyan!40!white,
%         draw=blue,
%         bar shift=.9
%         % opacity=.4
%     ] table [x index=0, y index=1] {data/min_constrastive_distances.txt};

%     \end{axis}
%     \end{tikzpicture}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

==> sections/our_policy_save2709.tex <==
In this paper, we propose a new hierarchical goal conditionned offline RL algorithm: Quantizing Planner for Hierarchical Implicit Q-Learning (QPHIL). 
%The design of QPHIL is inspired by how humans naturally describe and plan trajectories. 
While current hierarchical methods rely heavily on continuous waypoint predictions, our approach is using more general subgoals, allowing to simplify the planning process. Instead of relying on precise coordinates, QPHIL identifies key landmarks to guide trajectory planning, much like how a road trip is described by cities or highways rather than specific geographic points. The algorithm detects these landmarks, creates landmark-based sequences, and formulates policies to navigate between them, ultimately reaching the target destination.

\subsection{Overall design}

QPHIL operates through three main components: a state quantizer, a sequence generator, and a policy module. The state quantizer is used to map raw states into discrete representations, referred to as tokens or landmarks, which serve as the building blocks for planning. These discrete representations are then processed by the sequence generator, which assembles them into a coherent sequence that outlines the overall trajectory to be followed. A graphical representation of the inference pipeline is available in~\Cref{fig:inf_pipeline} and the pseudo-code in~\Cref{alg:qphil}.

To execute the plan, QPHIL uses two policies. The first policy navigates between these discrete representations, effectively moving from one identified landmark to the next in the sequence. After the sequence has been executed, a second policy is used to reach the goal within the last landmark.

\input{inference_pipeline}

This method is hierarchical. The sequence generator is effectively the high level policy and the two navigation policies are the low level policies. Unlike most hierarchical methods that invoke the high-level policy at each step, QPHIL generates the entire plan in a single step, creating a coherent sequence of landmarks that effectively guides the agent towards its goal.



\subsection{Tokenization}

Discrete state tokens are learnt using a Vector Quantized-Variational AutoEncoder (VQ-VAE)~\cite{oord2018neural}, \textit{i.e.} an autoencoder with a finite latent space.
%A VQ-VAE is an autoencoder with a finite latent space, meaning that when a deterministic decoder is used, the output space also remains finite. This results in a well-defined set of tokens, where the VQ-VAE effectively maps states to their corresponding tokens.\\
% We considered several alternatives for tokenization, including DINO~\cite{caron2021emerging}, encoding the space to a sphere followed by K-means clustering, and manual segmentation using either a uniform grid or quantiles, as seen in Trajectory Transformer~\cite{janner2021offline}. However, we chose to use VQ-VAE for its simplicity and its ability to learn meaningful representations that we believe could generalize better. The implementation was straightforward, and initial results were promising, which reinforced our decision to keep this method.\\
The use of VQ-VAE for tokenization has been proposed in various domains, including time series analysis~\cite{lee2024leveraging}, video pretraining~\cite{tan2021vimpac}, and vision transformers~\cite{dong2023peco}; it has also been explored in offline reinforcement learning~\cite{jiang2022efficient, sudhakaran2023skill}. However, to the best of our knowledge, this type of tokenization has not been previously applied in planning.

% In simpler scenarios, this tokenization step could be replaced by a more straightforward, scripted approach (e.g., a grid for navigation). Nonetheless, our proposed method offers an automated solution that is particularly useful in cases where tokenization is not intuitive or where the state space is too large and complex.\\

The tokenizer is composed of three main elements (see~\Cref{fig:tokenization-pipeline}): an encoder, a quantizer, and a decoder. The encoder maps the state space to a latent space, the quantizer maps the latent space to a finite set of tokens, and the decoder maps the tokens back to the state space.

A reconstruction loss is typically used to train a VQ-VAE. However, in the context of offline reinforcement learning, this loss alone is insufficient to achieve meaningful tokenization. The reason is that two states can be numerically close but very different in their meaning in terms of RL. For instance, two positions on either side of a wall might be numerically close in a model that is map-agnostic, yet they represent entirely different scenarios in terms of trajectory planning.% This issue becomes particularly problematic in HIQL when the walls are thin, which is precisely the challenge our proposed method aims to address.

\input{figures/thin_walls}

In offline reinforcement learning, temporal proximity is more important than spatial proximity. Therefore, it has been proposed to use a contrastive loss to ensure that temporally close states are assigned the same tokens, while temporally distant states receive different tokens. To achieve this, we use the triplet margin loss~\citep{balntas2016learning}:
\[
    \mathcal L_\text{contrastive} = \mathbb E_{\substack{s_t \sim \mathcal D\\ k \sim \inte {-\omega} {\omega} \\ k' \sim \Z \backslash \inte {-\omega} {\omega} }} \max\left\{d(g(s_{t}), g(s_{t + k})) - d(g(s_{t}), g(s_{t + k'})), 0 \right\}, 
\]
where \(\mathcal D\) is the dataset, \(g\) is the encoder, \(d\) is the Euclidean norm and \(\omega\) is the time window used to define what is a close state.

To help the VQ-VAE learn a meaningful representation, a reconstruction loss is used. This ensures the model get close to the identity function, despite the finite output space:
\[
    \mathcal L_\text{recon} = \mathbb E_{s \sim \mathcal D}||T(s) - s||_2^2,
\] where \(\mathcal D\) is the dataset and \(T\) is the complete tokenizer.

As explained by authors of the VQ-VAE architecture~\citep{van2017neural}, the embedding space grows arbitrarily if the embedding does not train as fast as the encoder parameters. The commitment loss is used to prevent this issue:
\[
    \mathcal L_\text{commit} = \mathbb E_{s \sim \mathcal D}||g(s) - \text{sg}(q(g(s))||_2^2 + \beta||\text{sg}(g(s)) - q(g(s))||_2^2,
\]
where sg is the stop-gradient operator, \(\beta\) is a hyperparameter, \(\mathcal D\) is the dataset, \(g\) is the generator and \(q\) is the quantizer.

\input{figures/tokenization_pipeline}

The tokenizer loss, used in training is then a linear combination of the three previous losses:
\[
    \mathcal L_\text{tokenizer} = \mathcal L_\text{recon} + \alpha_1 \mathcal L_\text{commit} + \alpha_2 \mathcal L_\text{contrastive}.
\]

An illustration of the training process is available in~\Cref{fig:tokenization-pipeline} and some examples of tokenization are shown in~\Cref{fig:tokenization-exemple}.
%This result correspond well to what we would have designed ourselves.
Clusters (zone associated to a given token) are smaller where data is abundant and larger where data is scarce. Trajectories of the dataset are somehow visible in the shapes of the clusters. 

\input{figures/tokenization_exemple}

The utility of the contrastive loss is perceivable in~\Cref{fig:tokenization-exemple_tokenization_exemple}. However, its strength is really revealed in~\Cref{fig:godot_tokenization_exemple}: walls are extremely thin and the tokenization completely take it into consideration. Clusters do not align perfectly with the walls, which we attribute to the scarcity of data near the wall.

\subsection{Sequence generation}

Once the tokenizer has been trained, states from dataset trajectories can be converted into sequences of discrete tokens, effectively transforming continuous state trajectories into symbolic sequences. The temporal contrastive loss used during training ensures consistency within these sequences, as depicted in~\Cref{fig:tokenization-pipeline}. This consistency manifests as repeated tokens for similar states within a given region. By applying a simple post-processing step that removes consecutive repetitions, we obtain a more concise sequence that succinctly represents the key zones to traverse in the correct order. 
For instance, a tokenized sequence such as ``1 1 1 2 2 3 3 3 4 4'' is simplified to ``1 2 3 4'', reflecting the core structure of the trajectory. This process is illustrated in~\Cref{fig:compression}. A new dataset \(\mathcal S\) of simplified sequences of tokens is then generated and used to train the sequence generator. Additional cleaning steps are described in~\Cref{subsection:data-cleaning}.

\input{figures/compression}

This dataset is used to train an encoder-decoder transformer model~\citep{vaswani2017attention}, which is a sequence-to-sequence model that is particularly well-suited for this task. The transformer is trained to predict the next token in the sequence given the previous tokens using the teacher forcing algorithm: at train time, given a sequence \((x_i)_{i < n}\) from the dataset, the model receives \(\left\{(x_i)_{i < m}\right\}_{m < n - 1}\). For each of these \(n\) beginning of sequence, the model generates a probability \((y_{i,j})_{j}\) for each token \(j\), where \(i\) is the index of the predicted element in the sequence. Output of the model is a probability distribution over tokens and we use the cross-entropy loss, which measures the difference between the predicted token probabilities and the actual tokens in the sequence:
\[
    \mathcal{L}_\text{transformer} = - \sum_{i=0}^{n-1} \log\dfrac{\exp x_{t, a_i}}{\sum_m \exp x_{i, m}}  ,
\]
where \(a_i\) is the actual token index for the element \(i\) of the sequence and for all \(j\), \(y_{i, j}\) is the predicted probability of the token \(m\) for the element \(i\).

In order to generate sequences that start from the initial position and end at the goal, the encoder of the transformer receives the goal token, a start of sequence token and then the initial token. 

During inference, the encoder is fed the input sequence. Then, until the model outputs the end of sequence token, the output of the encoder and previously generated tokens (none at the first step) are fed to the decoder. A softmax layer and a temperature parameter \(T\) are then used on the output of the decoder to create a distribution over the tokens. The token is then sampled from this distribution:
\[
    y_t \sim \text{Cat}\left(\dfrac{\exp\left(\dfrac{z^i_t}{T}\right)}{\sum_{j}\exp\left(\dfrac{z^j_{t}}{T}\right)} \right)_i,
\] 
where \(z_t\) is the output of the decoder at step \(t\). This process is repeated until the model outputs the end of sequence token. Pseudo-code of the inference is available in~\Cref{alg:inference_transformer}.

% \input{sequence_generation}

\subsubsection{Data augmentation}\label{sec:data-augmentation}


One of the most crucial aspects of offline reinforcement learning is stitching. Incorporating it in the training part is not easy for most algorithms when the data is continuous as one exact state is unlikely to be repeated. However, in our case, we have a discrete representation of the state space, which means that states (here tokens) are repeated often. This allows us to use data augmentation techniques that are not possible in continuous spaces.

\input{stitching}

We propose to use a simple data augmentation technique: for each pair of sequence, if the final token of the first sequence is in the second one, we add a new trajectory in the dataset: the first sequence followed by the end of the second one.
%We could generate a lot more data by considering all tokens from the first sequence instead. However, using only the last one generate enough new data to be useful and is much faster. 
%It also helps to keep a balance between the number of real sequences and generated ones.
This technique is illustrated in~\Cref{fig:data_augmentation}. We leave the design and analysis of more complex stitching mechanisms for future work. 
% While we create many more sequences\footnote{The dataset size can be multiplied by a factor of 10.}, it can easily be implemented in a data efficient way. The pair of sequences and stitching index are stores and concatenation is done on the fly. This could allow more data generation by considering more than the last index of the first sequence or by successively stitching sequences from stitched sequences.



\subsection{Actual policy}

The final component of our algorithm is the policy that learns action execution. This policy approximates the distribution \(\pi(a | s, g)\), where \(a\) is an action form that dataset associated with a state \(s\) and either a goal or a subgoal \(g\). Initially, we attempted to develop a single unified policy for both goals and subgoals. However, this approach underperformed, leading us to adopt two separate policies. The first, the ``goal policy'' takes the current state and goal as input and outputs a distribution of actions, trained using the standard IQL algorithm. The second, the ``subgoal policy'' is a variant of IQL adapted for subgoal-directed tasks.

Although it might seem intuitive to train the subgoal policy using IQL with a token representation of the goal, this introduces unnecessary complexity without providing significant benefits. At inference time, the subgoal policy has to the next subgoal, which corresponds to a neighboring token. Training the policy to reach long-term goals would undermine the planner, wasting resources and potentially degrading performance. Instead, during training, the goal provided to the subgoal policy is the next token in the episode’s token sequence, aligning with the inference process.

While both HIQL and QPHIL are hierarchical extensions of IQL, their high-level policies differ significantly. HIQL uses the same value function for both its high and low-level policies. Although using a shared value function for our two policies would have been more elegant, the disparity in goal representations made it impractical.



==> sections/our_policy_save2909.tex <==
In this paper, we propose a new hierarchical goal conditionned offline RL algorithm: Quantizing Planner for Hierarchical Implicit Q-Learning (QPHIL). 
%The design of QPHIL is inspired by how humans naturally describe and plan trajectories. 
While current hierarchical methods rely heavily on continuous waypoint predictions, we propose to consider discrete subgoals, allowing to simplify the planning process. Instead of relying on precise coordinates, QPHIL identifies key landmarks to guide trajectory planning, much like how a road trip is described by cities or highways rather than specific geographic points. The algorithm detects these landmarks, creates landmark-based sequences, and formulates policies to navigate between them, ultimately reaching the target destination.

\subsection{Overall design}

QPHIL operates through four components: a state quantizer \(\phi\), which divides the state set into a finite set of landmarks, a plan generator $\pi^{plan}$, which acts as a high-level policy to generate a sequence of landmarks to be reached given the final goal, and two low-level policy modules: \(\pi^\text{landmark}\), which targets state areas defined as landmarks, and \(\pi^\text{goal}\), which targets a specific state goal. 

\begin{wrapfigure}{l}{.4\textwidth}
    \centering
    \begin{tikzpicture}[
        node distance=.3cm, 
        every node/.style={fill=white, font=\scriptsize}, 
        encoder/.style={trapezium, trapezium angle=70, draw=yellow!70!black, minimum width=1cm, minimum height=.75cm, rounded corners=.5pt, thick, fill=yellow!10},
        decoder/.style={trapezium, trapezium angle=110, draw=yellow!70!black, minimum width=1 cm, minimum height=.75cm, rounded corners=.5pt, thick, fill=yellow!10},
        latent/.style={rectangle, draw, rounded corners=.5pt, thick},
        loss/.style={rectangle, draw, rounded corners=2.5pt, draw=cyan!70!black, thick, fill=cyan!10},
        rect/.style={rectangle, draw, rounded corners=2.5pt, thick},
        codebook/.style={matrix of nodes, nodes={draw, rectangle, minimum width=0.25cm, minimum height=0.5cm, anchor=center}, rounded corners=.5pt, thick},
        arrow/.style={-Stealth}
    ]
        \node[fill=none] (s0) {\(s_0\)};
        \node[fill=none, left=of s0] (g) {\(g\)};
        \begin{scope}[on background layer]
            \node[fit=(g.north west) (s0.south east), fill=gray!10, draw=gray!70!black, thick, rounded corners=2.5pt] (rectangle) (input) {};
        \end{scope}

        \node[rect, below=.5cm of s0.south east] (tokenizer) {Tokenizer};

        \node[rect, below=1cm of tokenizer] (transformer) {Transformer};

        \coordinate (midpoint) at ($(tokenizer)!0.5!(transformer)$);
        \node[fill=none] at ($(midpoint) - (1,0)$) (token_s0) {Token \(s_0\)};
        \node[fill=none] at ($(midpoint) + (1,0)$) (token_g) {Token \(g\)};
        \begin{scope}[on background layer]
            \node[fit=(token_s0.north west) (token_g.south east), fill=purple!10, draw=purple!70!black, thick, rounded corners=2.5pt] (rectangle) at (midpoint) (tokens) {};
        \end{scope}

        \node[rect, below=of transformer] (subgoals) {Subgoal sequence};
        \node[fill=none, left=.5cm of subgoals] (token_left) {\footnotesize{Token left ?}};
        \node[fill=none, below=of token_left] (no) {\footnotesize{No}};
        \node[fill=none, right=of no] (yes) {\footnotesize{Yes}};
        \node[fill=none, above=of token_left] (sk) {\(s_k\)};

        \node[rect, below=of subgoals, draw=purple!70!black, fill=gray!10] (subgoal) {Next token};

        \node[rect, below=of subgoal, draw=cyan!70!black, fill=cyan!10] (subgoal_policy) {IQL Subgoal};
        \node[rect, left=of subgoal_policy, below=of no, draw=cyan!70!black, fill=cyan!10] (goal_policy) {IQL};

        \begin{scope}[on background layer]
            \node[fit=(subgoals.north east) ($(token_left.west |- goal_policy.south)$), fill=yellow!10, draw=yellow!70!black, thick, rounded corners=2.5pt] (rectangle) at ($(subgoals.east |- subgoal_policy.south)!.5!(token_left.north west)$) (dual_policy) {};
        \end{scope}

        \node[fill=none, below=of dual_policy] (action) {Action};


        \draw[arrow] (input) -- (tokenizer);

        \draw[arrow] (tokenizer) -- (token_s0);
        \draw[arrow] (tokenizer) -- (token_g);

        \draw[arrow] (token_s0) -- (transformer);
        \draw[arrow] (token_g) -- (transformer);

        \draw[arrow] (transformer) -- (subgoals);

        \draw[arrow] ($(subgoals.south) - (.25cm, 0)$) -- ($(subgoal.north) - (.25cm, 0)$);
        \draw[arrow] ($(subgoal.north) + (.25cm, 0)$) -- ($(subgoals.south) + (.25cm, 0)$);
        \draw[arrow] (subgoal) -- (subgoal_policy);

        % \draw[arrow] (g.south) to[in=90, out=-90] ($(tokens.west) - (.25cm, 0)$) to[out=-90, in=20] ($(($(tokens.west) - (.25cm, 0)$) |- dual_policy.north)$);
        \coordinate (intermediate) at ($(tokens.west) + (-0.25cm, 0)$);
        % \coordinate (intermediate1) at (intermediate |- dual_policy.north);
        \draw[arrow] (g.south) 
        to[in=90, out=-90] (intermediate) 
        to[out=-90, in=90] (intermediate |- dual_policy.north);

        \draw[arrow, thick] (sk) -- (token_left);
        \draw[arrow] (token_left) -- (yes);
        \draw[arrow] (token_left) -- (no);
        \draw[arrow, thin] (token_left) -- (subgoals);
        \draw[arrow, thin] (subgoals) -- (token_left);
        \draw[arrow] (yes) -- (subgoal);
        \draw[arrow] (no) -- (goal_policy);

        \draw[arrow, thick] (dual_policy) -- (action);

    \end{tikzpicture}
    \caption{Inference pipeline of QPHIL.}
    \label{fig:inf_pipeline}
\end{wrapfigure}

The state quantizer \(\phi: {\cal S} \to \Omega\), with \(\Omega \equiv  \inte{1}{k}\),   %$
is used to map raw states into a set of $k$ landmark indexes (or tokens), %, each associated to a continuous embedding defined in a learned code-book $z:[[1,k]] \rightarrow \mathbb{R}^d$. We denote as $z_{\omega}=z(\omega)$ the embedding associated with token $\omega$ in that code-book. % 
 which serve as the building blocks for our planning strategy. These discrete representations are then processed by the plan generator, which assembles them into a coherent sequence that outlines the overall trajectory to be followed in the environment to reach the  requested goal \(g\). Given %depending
 any history of tokens \((\omega_0,\cdots,\omega_s)_{s > 0}\) and a targeted goal \(g \in {\cal G}\), % to be reached for the task at end%that quantizer, 
%the $z:[[1,k]] \rightarrow \mathbb{R}^d$ 
the plan generator produces sequences of tokens \((\omega_{s+1},\cdots,\omega_{s+l})\) auto-regressively until \(\omega_{s+l}=\dot{\omega}\) (with \(\dot{\omega}\) an extra end of sequence token that stops the generation), following: $\pi^\text{plan}\left((\omega_{s+1},\cdots,\omega_{s+l})\ |\ \phi(g), (\omega_i)_{i=0}^{s}\right)=\prod_{t=1}^l \pi^\text{plan}\left(\omega_{s+t}\ |\ \phi(g), (\omega_i)_{i=0}^{s+l-1}\right)$.  %$ \times \pi^{plan}(\dot{\omega}|\phi(g), (\omega_i)_{i=0}^{s+l})$, with $\dot{\omega}$ an extra index corresponding to the end of sequence token that stops generation.
It is used from the start token \(\omega_0=\phi(s_0)\) of the episode,  to propose a sequence of landmarks to follow using \(\pi^\text{landmark}: {\cal A} \times {\cal S} \times \Omega \to [0,1]\), before navigating through the final goal \(g\) using \(\pi^\text{goal}: {\cal A} \times {\cal S} \times {\cal G} \to [0,1]\). Optionally, it can also be used to re-plan after a given condition is reached (e.g. every \(n\) steps or when the agent leaves its current area), which is mostly useful for complex environments with stochasticity.    

\Cref{alg:qphil_inference} presents the inference pseudo-code of our QPHIL approach. For a given goal \(g\) and a start state \(s_0\), the process first samples a new plan, which corresponds to a sequence of landmarks to be reached sequentially before driving towards \(g\).  Then, until the first subgoal \(\omega\) of this sequence is reached (which happens when \(\phi(s)=\omega\)), \(\pi^\text{landmark}\) is used conditioned on the current state and the sub-goal \(\omega\) to sample actions to emit in the environment. When the sub-goal is reached, it is removed from the list, and we move to the next one, and so on until the list of sub-goals is empty. At that point, we should be ready to apply \(\pi^\text{goal}\) to move on toward the requested goal \(g\). A graphical representation of the inference pipeline is available in~\Cref{fig:inf_pipeline}. % and the pseudo-code in~\Cref{alg:qphil}. 


%of  discrete representations, referred to as tokens or landmarks, which serve as the building blocks for planning. These discrete representations are then processed by the sequence generator, which assembles them into a coherent sequence that outlines the overall trajectory to be followed. A graphical representation of the inference pipeline is available in~\Cref{fig:inf_pipeline} and the pseudo-code in~\Cref{alg:qphil}.

%To execute the plan, QPHIL uses two policies. The first policy navigates between these discrete representations, effectively moving from one identified landmark to the next in the sequence. After the sequence has been executed, a second policy is used to reach the goal within the last landmark.

\begin{algorithm}[H]
    \caption{\label{alg:qphil_inference}  Navigation with QPHIL}
    \begin{algorithmic}
    
    
    \Require Goal state \(g\), Start state \(s_0\), State quantizer \(\phi\), Sequence generator \(\pi^{plan}\), Navigation policies \(\pi^{\text{landmark}}\) and \(\pi^{\text{goal}}\)
    %\Ensure Action \(a\) to reach \(g\) from \(s\)
    \State \(\tau^< = (\phi(s_0))\); \(\tau^>=\{\}\);   \(s=s_0\); 
    \While{Not exceeding a  max number of steps} %$g$ is not reached (and not exceeding a  max number of steps)}
    \If{First step (or if re-planning is required)}% $\qquad$ \textit{   // Generate  future landmarks }
    \Comment{Generate  future landmarks}
        %\State 
        \State \(\tau^> \gets  (\omega_{1},\omega_{2},\dots, \dot{\omega}) \sim \pi^\text{plan}(.\ |\ \phi(g), \tau^<)\) %\mathcal{L} \gets G_{\text{seq}}(z_0, z_G)\)
    \EndIf
    
    %\If{\(\tau^>\) is not empty}
    \If{$\tau^>_0 \ != \ \dot{\omega}$}
        \(a \sim \pi^{\text{landmark}}(.\ |\ s, \tau^>_0)\)
    \Else\  \(a \sim \pi^{\text{goal}}(.\ |\ s, g)\)
    \EndIf
    \State Emit \(a\) in the environment and observe new state \(s'\)
    \State \(s \gets s'\); 
    %\If{\(\tau^>\) is not empty}
    \If{$\tau^>_0 \ != \ \dot{\omega}$}  
        \If{\(\phi(s)==\tau^>_0\)} %$\qquad \qquad \qquad \qquad$ \textit{   // Subgoal  reached, go to the next one}
        \Comment{Subgoal  reached, go to the next one}
        \State $\tau^<.\text{append}(\tau^>.\text{pop}(0))$; 
        \EndIf
    \Else\  
        \If{\(s\) is in \(g\)}  %$\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad$ \textit{    // Final goal  reached}
        \Comment{Final goal  reached}
            \State return;     
        \EndIf
    \EndIf
    
    
    
    \EndWhile
    %\Return \(a\)
    \end{algorithmic}
\end{algorithm}

% \input{inference_pipeline}

%This method is hierarchical. The sequence generator is effectively the high level policy and the two navigation policies are the low level policies. Unlike most hierarchical methods that invoke the high-level policy at each step, QPHIL generates the entire plan in a single step, creating a coherent sequence of landmarks that effectively guides the agent towards its goal.



The remainder of this section presents our learning methodology for every component of our QPHIL approach. 

\subsection{Tokenization}

\begin{wrapfigure}[17]{r}{.4\textwidth}
    \centering
        \vspace{-.73cm}
        \includegraphics[width=.4\textwidth]
        {figures/background_tokens_utra.pickle}
        \vspace{-.6cm}
        
        % \caption{Antmaze Ultra}
        \label{fig:tokenization-exemple_tokenization_exemple}
    \caption{Tokenization example. Each token has an associated color. The color of each point in the background correspond to the color of the associated token. It is noticeable that the tokens align with the walls thanks to the contrastive loss.}
\end{wrapfigure}

Discrete state tokens are learnt using a Vector Quantized-Variational AutoEncoder (VQ-VAE)~\cite{oord2018neural}, \textit{i.e.} an autoencoder with a finite latent space.
%A VQ-VAE is an autoencoder with a finite latent space, meaning that when a deterministic decoder is used, the output space also remains finite. This results in a well-defined set of tokens, where the VQ-VAE effectively maps states to their corresponding tokens.\\
% We considered several alternatives for tokenization, including DINO~\cite{caron2021emerging}, encoding the space to a sphere followed by K-means clustering, and manual segmentation using either a uniform grid or quantiles, as seen in Trajectory Transformer~\cite{janner2021offline}. However, we chose to use VQ-VAE for its simplicity and its ability to learn meaningful representations that we believe could generalize better. The implementation was straightforward, and initial results were promising, which reinforced our decision to keep this method.\\
The use of VQ-VAE for tokenization has been proposed in various domains, including time series analysis~\cite{lee2024leveraging}, video pretraining~\cite{tan2021vimpac}, and vision transformers~\cite{dong2023peco}; it has also been explored in offline reinforcement learning~\cite{jiang2022efficient, sudhakaran2023skill}. However, to the best of our knowledge, this type of tokenization has not been previously applied in planning.

% In simpler scenarios, this tokenization step could be replaced by a more straightforward, scripted approach (e.g., a grid for navigation). Nonetheless, our proposed method offers an automated solution that is particularly useful in cases where tokenization is not intuitive or where the state space is too large and complex.\\
% \input{figures/tokenization_exemple}


As defined in previous section, the state quantizer \(\phi\) %: {\cal S} \to \Omega\), with \(\Omega \equiv  \inte{1}{k}\),   %$
is used to map raw states into a set of $k$ tokens. It is composed of a state encoder $g: {\cal S} \rightarrow \mathbb{R}^d$, which maps the state space to a latent space of dimension $d$, and a learned code-book $z:\Omega  \rightarrow \mathbb{R}^d$, which  associates each token to a continuous embedding. %We denote as $z_{\omega}=z(\omega)$ the embedding associated with token $\omega$ in that code-book. % 
% which serve as the building blocks for our planning strategy.
From these, $\phi$ is defined as: $\phi(s)=\arg\min_{\omega \in \Omega} \Delta(g(s),z(\omega))$, with $\Delta$ the euclidean distance in the latent space.   


%The tokenizer is composed of three main elements: an encoder $g: {\cal S} \rightarrow \mathbb{R}^d$, a  \(\phi: {\cal S} \to \Omega\), with \(\Omega \equiv  \inte{1}{k}\), and a decoder $f: \mathbb{R}^d \rightarrow {\cal S}$. The encoder maps the state space to a latent space, the quantizer maps the latent space to a finite set of tokens, and the decoder maps the tokens back to the state space. 
As depicted in Figure~\Cref{fig:tokenization-pipeline}, three losses are considered to train these components. First, the VQ-VAE learns a meaningful representation by considering a reconstruction loss, which ensures that states can be decoded from tokens they are projected into:  % It ensures that tokens encode can be decoded to input states that are the input state can be decoded from the model gets close to the identity function, despite the finite output space:
\[
    \mathcal L_\text{recon} = \mathbb E_{s \sim \mathcal D}||f(z(\phi(s))) - s||_2^2,
\] where \(\mathcal D\) is the dataset and \(f: \mathbb{R}^d \rightarrow {\cal S}\) is a decoder network trained together with the code-book of token embeddings. 

As the gradient flow stops in the previous loss due to the discrete projection performed by $\phi$, we need to consider an additional commitment loss to learn the encoder parameters: 
\[
    \mathcal L_\text{commit} = \mathbb E_{s \sim \mathcal D}||g(s) - \text{sg}(z(\phi(s))||_2^2 + \beta||\text{sg}(g(s)) - z(\phi(s))||_2^2,
\]
where sg is the stop-gradient operator. The first term of this loss aims at attracting %latent encodings of states getting closer 
encoder  outputs close to the  code of the token states project into. %The second term, weighted by a hyperparameter \(\beta\), aims % is , \(\mathcal D\) is the dataset, \(g\) is the generator and \(q\) is the quantizer.
%
%that  
%
As explained by authors of the VQ-VAE architecture~\citep{van2017neural}, the embedding space grows arbitrarily if the token embedding does not train as fast as the encoder parameters. The second term, weighted by a hyperparameter \(\beta\), aims to prevent this issue. 

%A reconstruction loss is typically used to train a VQ-VAE. However, i
%In the context of offline reinforcement learning, this loss alone is insufficient to achieve meaningful tokenization. The reason is that two states can be numerically close but very different in their meaning in terms of RL. For instance, two positions on either side of a wall might be numerically close in a model that is map-agnostic, yet they represent entirely different scenarios in terms of trajectory planning.% This issue becomes particularly problematic in HIQL when the walls are thin, which is precisely the challenge our proposed method aims to address.

%\input{figures/thin_walls}

To introduce dynamics of the environment in the representation learned, we consider a third contrastive loss 
%
%
%In offline reinforcement learning, temporal proximity is more important than spatial proximity. Therefore, it has been proposed to use a contrastive loss
that incentivize temporally close states to be  assigned the same tokens, while temporally distant states receive different tokens. To achieve this, we use the triplet margin loss~\citep{balntas2016learning} applied to our setting:
\[
    \mathcal L_\text{contrastive} = \mathbb E_{\substack{s_t \sim \mathcal D\\ k \sim \inte {-\gamma} {\gamma} \\ k' \sim \Z \backslash \inte {-\gamma} {\gamma} }} \max\left\{\Delta(g(s_{t}), g(s_{t + k})) - d(g(s_{t}), g(s_{t + k'})), 0 \right\}, 
\]
where %\(\mathcal D\) is the dataset, \(g\) is the encoder, \(d\) is the Euclidean norm and \
\(\gamma\) is the time window used to specify temporal closeness of states in demonstration trajectories. %define what is a close state.
This loss is for instance of crucial importance in navigation settings with thin walls, where two states can be close in the input space, while corresponding to very different situations. 

The tokenizer loss, used in training is then a linear combination of the three previous losses:
\[
    \mathcal L_\text{tokenizer} = \mathcal L_\text{recon} + \alpha_1 \mathcal L_\text{commit} + \alpha_2 \mathcal L_\text{contrastive}.
\]

An illustration of the training process is available in~\Cref{fig:tokenization-pipeline} and some examples of tokenization are shown in~\Cref{fig:tokenization-exemple}.
%This result correspond well to what we would have designed ourselves.
Clusters (zone associated to a given token) are smaller where data is abundant and larger where data is scarce. Trajectories of the dataset are somehow visible in the shapes of the clusters. 


%The utility of the contrastive loss is perceivable in~\Cref{fig:tokenization-exemple_tokenization_exemple}. However, its strength is really revealed in~\Cref{fig:godot_tokenization_exemple}: walls are extremely thin and the tokenization completely take it into consideration. Clusters do not align perfectly with the walls, which we attribute to the scarcity of data near the wall.

\subsection{Sequence generation}

Once the tokenizer has been trained, states from dataset trajectories can be converted into sequences of discrete tokens, effectively transforming continuous state trajectories into symbolic sequences. The temporal contrastive loss used during training ensures consistency within these sequences, as depicted in~\Cref{fig:tokenization-pipeline}. This consistency manifests as repeated tokens for similar states within a given region. By applying a simple post-processing step $\eta^\phi(\tau)$ that removes consecutive repetitions of tokens in a trajectory $\tau$, we obtain a more concise sequence that succinctly represents the key zones to traverse in the correct order. 
For instance, a tokenized sequence such as ``1 1 1 2 2 3 3 3 4 4'' is simplified to ``1 2 3 4'', reflecting the core structure of the trajectory. This process is illustrated in~\Cref{fig:compression}.

%A new dataset \(\mathcal S\) of simplified sequences of tokens is then generated and used to train the sequence generator. Additional cleaning steps are described in~\Cref{subsection:data-cleaning}.

\input{figures/compression}

%This dataset is used to train an encoder-decoder transformer model~\citep{vaswani2017attention}, which is a sequence-to-sequence model that is particularly well-suited for this task. The transformer is trained to predict the next token in the sequence given the previous tokens using the teacher forcing algorithm: at train time, given a sequence \((x_i)_{i < n}\) from the dataset, the model receives \(\left\{(x_i)_{i < m}\right\}_{m < n - 1}\). For each of these \(n\) beginning of sequence, the model generates a probability \((y_{i,j})_{j}\) for each token \(j\), where \(i\) is the index of the predicted element in the sequence. Output of the model is a probability distribution over tokens and we use the cross-entropy loss, which measures the difference between the predicted token probabilities and the actual tokens in the sequence:
Then, the planner $\pi^{plan}$ is trained following a teacher forcing approach on trajectories from ${\cal D}$:
\[
    \mathcal{L}_\text{plan} = - \mathbb{E}_{s\sim {\cal D}} \quad \mathbb{E}_{\hspace{-0.5cm}\substack{t<|\tau|,\\\phi(\tau_t) \neq \phi(\tau_{t+1})}} % (\omega,\omega'), \\ \exists t \phi(\tau_t)=\omega \\ \wedge 
 %\phi(\tau_{t+1})=\omega'}}
 \log \pi^{plan}(\phi(\tau_{t+1})|\phi(g),\eta^\phi(\tau_{\leq t})) ,
\]
with $|\tau|$ the number of states in $\tau$, $\tau_t$ the $t$-th state in $\tau$, and $\tau_{\leq t}$ the history of $\tau$ at step $t$. 
We implement $\pi^{plan}$ using a %n encoder-decoder 
transformer architecture~\citep{vaswani2017attention} $h_\theta$, where $\pi^{plan}(.|\phi(g),\eta^\phi(\tau_{\leq t}))$ is defined for any $\omega \in \Omega$ using a softmax on the outputs of $h_\theta(\phi(g),\eta^\phi(\tau_{\leq t}))$. 


%\[
%    \mathcal{L}_\text{transformer} = - \sum_{i=0}^{n-1} \log\dfrac{\exp x_{t, a_i}}{\sum_m \exp x_{i, m}}  ,
%\]
%where \(a_i\) is the actual token index for the element \(i\) of the sequence and for all \(j\), \(y_{i, j}\) is the predicted probability of the token \(m\) for the element \(i\).

%In order to generate sequences that start from the initial position and end at the goal, the encoder of the transformer receives the goal token, a start of sequence token and then the initial token. 

%During inference, the encoder is fed the input sequence. Then, until the model outputs the end of sequence token, the output of the encoder and previously generated tokens (none at the first step) are fed to the decoder. A softmax layer and a temperature parameter \(T\) are then used on the output of the decoder to create a distribution over the tokens. The token is then sampled from this distribution:
%\[
%    y_t \sim \text{Cat}\left(\dfrac{\exp\left(\dfrac{z^i_t}{T}\right)}{\sum_{j}\exp\left(\dfrac{z^j_{t}}{T}\right)} \right)_i,
%\] 
%where \(z_t\) is the output of the decoder at step \(t\). This process is repeated until the model outputs the end of sequence token. Pseudo-code of the inference is available in~\Cref{alg:inference_transformer}.

% \input{sequence_generation}


\subsection{Low-level policies}

%The final component of our algorithm is the policy that learns action execution. This policy approximates the distribution \(\pi(a | s, g)\), where \(a\) is an action form that dataset associated with a state \(s\) and either a goal or a subgoal \(g\). Initially, we attempted to develop a single unified policy for both goals and subgoals. However, this approach underperformed, leading us to adopt two separate policies. The first, the ``goal policy'' takes the current state and goal as input and outputs a distribution of actions, trained using the standard IQL algorithm. The second, the ``subgoal policy'' is a variant of IQL adapted for subgoal-directed tasks.

As described above, two low-level policies $\pi^{lamndmark}$ and $\pi^{goal}$ have to be trained to perform actions in the environment. 

Donner l'equation d'apprentissage IQL appliqué a ces deux politiques

%Although it might seem intuitive to train the subgoal policy using IQL with a token representation of the goal, this introduces unnecessary complexity without providing significant benefits. At inference time, the subgoal policy has to the next subgoal, which corresponds to a neighboring token. Training the policy to reach long-term goals would undermine the planner, wasting resources and potentially degrading performance. Instead, during training, the goal provided to the subgoal policy is the next token in the episode’s token sequence, aligning with the inference process.

%While both HIQL and QPHIL are hierarchical extensions of IQL, their high-level policies differ significantly. HIQL uses the same value function for both its high and low-level policies. Although using a shared value function for our two policies would have been more elegant, the disparity in goal representations made it impractical.



\subsubsection{Data augmentation}\label{sec:data-augmentation}


One of the most crucial aspects of offline reinforcement learning is stitching. Incorporating it in the training part is not easy for most algorithms when the data is continuous as one exact state is unlikely to be repeated. However, in our case, we have a discrete representation of the state space, which means that states (here tokens) are repeated often. This allows us to use data augmentation techniques that are not possible in continuous spaces.

\input{stitching}

We propose to use a simple data augmentation technique: for each pair of sequence, if the final token of the first sequence is in the second one, we add a new trajectory in the dataset: the first sequence followed by the end of the second one.
%We could generate a lot more data by considering all tokens from the first sequence instead. However, using only the last one generate enough new data to be useful and is much faster. 
%It also helps to keep a balance between the number of real sequences and generated ones.
This technique is illustrated in~\Cref{fig:data_augmentation}. We leave the design and analysis of more complex stitching mechanisms for future work. 
% While we create many more sequences\footnote{The dataset size can be multiplied by a factor of 10.}, it can easily be implemented in a data efficient way. The pair of sequences and stitching index are stores and concatenation is done on the fly. This could allow more data generation by considering more than the last index of the first sequence or by successively stitching sequences from stitched sequences.





==> sections/our_policy_save3009_13h.tex <==
In this paper, we propose a new hierarchical goal conditionned offline RL algorithm: Quantizing Planner for Hierarchical Implicit Q-Learning (QPHIL). 
%The design of QPHIL is inspired by how humans naturally describe and plan trajectories. 
While current hierarchical methods rely heavily on continuous waypoint predictions, we propose to consider discrete subgoals, allowing to simplify the planning process. Instead of relying on precise coordinates, QPHIL identifies key landmarks to guide trajectory planning, much like how a road trip is described by cities or highways rather than specific geographic points. The algorithm detects these landmarks, creates landmark-based sequences, and formulates policies to navigate between them, ultimately reaching the target destination.

\subsection{Overall design}

QPHIL operates through four components: a state quantizer \(\phi\), which divides the state set into a finite set of landmarks, a plan generator $\pi^{plan}$, which acts as a high-level policy to generate a sequence of landmarks to be reached given the final goal, and two low-level policy modules: \(\pi^\text{landmark}\), which targets state areas defined as landmarks, and \(\pi^\text{goal}\), which targets a specific state goal. 

\begin{wrapfigure}{l}{.4\textwidth}
    \centering
    \begin{tikzpicture}[
        node distance=.3cm, 
        every node/.style={fill=white, font=\scriptsize}, 
        encoder/.style={trapezium, trapezium angle=70, draw=yellow!70!black, minimum width=1cm, minimum height=.75cm, rounded corners=.5pt, thick, fill=yellow!10},
        decoder/.style={trapezium, trapezium angle=110, draw=yellow!70!black, minimum width=1 cm, minimum height=.75cm, rounded corners=.5pt, thick, fill=yellow!10},
        latent/.style={rectangle, draw, rounded corners=.5pt, thick},
        loss/.style={rectangle, draw, rounded corners=2.5pt, draw=cyan!70!black, thick, fill=cyan!10},
        rect/.style={rectangle, draw, rounded corners=2.5pt, thick},
        codebook/.style={matrix of nodes, nodes={draw, rectangle, minimum width=0.25cm, minimum height=0.5cm, anchor=center}, rounded corners=.5pt, thick},
        arrow/.style={-Stealth}
    ]
        \node[fill=none] (s0) {\(s_0\)};
        \node[fill=none, left=of s0] (g) {\(g\)};
        \begin{scope}[on background layer]
            \node[fit=(g.north west) (s0.south east), fill=gray!10, draw=gray!70!black, thick, rounded corners=2.5pt] (rectangle) (input) {};
        \end{scope}

        \node[rect, below=.5cm of s0.south east] (tokenizer) {Tokenizer};

        \node[rect, below=1cm of tokenizer] (transformer) {Transformer};

        \coordinate (midpoint) at ($(tokenizer)!0.5!(transformer)$);
        \node[fill=none] at ($(midpoint) - (1,0)$) (token_s0) {Token \(s_0\)};
        \node[fill=none] at ($(midpoint) + (1,0)$) (token_g) {Token \(g\)};
        \begin{scope}[on background layer]
            \node[fit=(token_s0.north west) (token_g.south east), fill=purple!10, draw=purple!70!black, thick, rounded corners=2.5pt] (rectangle) at (midpoint) (tokens) {};
        \end{scope}

        \node[rect, below=of transformer] (subgoals) {Subgoal sequence};
        \node[fill=none, left=.5cm of subgoals] (token_left) {\footnotesize{Token left ?}};
        \node[fill=none, below=of token_left] (no) {\footnotesize{No}};
        \node[fill=none, right=of no] (yes) {\footnotesize{Yes}};
        \node[fill=none, above=of token_left] (sk) {\(s_k\)};

        \node[rect, below=of subgoals, draw=purple!70!black, fill=gray!10] (subgoal) {Next token};

        \node[rect, below=of subgoal, draw=cyan!70!black, fill=cyan!10] (subgoal_policy) {IQL Subgoal};
        \node[rect, left=of subgoal_policy, below=of no, draw=cyan!70!black, fill=cyan!10] (goal_policy) {IQL};

        \begin{scope}[on background layer]
            \node[fit=(subgoals.north east) ($(token_left.west |- goal_policy.south)$), fill=yellow!10, draw=yellow!70!black, thick, rounded corners=2.5pt] (rectangle) at ($(subgoals.east |- subgoal_policy.south)!.5!(token_left.north west)$) (dual_policy) {};
        \end{scope}

        \node[fill=none, below=of dual_policy] (action) {Action};


        \draw[arrow] (input) -- (tokenizer);

        \draw[arrow] (tokenizer) -- (token_s0);
        \draw[arrow] (tokenizer) -- (token_g);

        \draw[arrow] (token_s0) -- (transformer);
        \draw[arrow] (token_g) -- (transformer);

        \draw[arrow] (transformer) -- (subgoals);

        \draw[arrow] ($(subgoals.south) - (.25cm, 0)$) -- ($(subgoal.north) - (.25cm, 0)$);
        \draw[arrow] ($(subgoal.north) + (.25cm, 0)$) -- ($(subgoals.south) + (.25cm, 0)$);
        \draw[arrow] (subgoal) -- (subgoal_policy);

        % \draw[arrow] (g.south) to[in=90, out=-90] ($(tokens.west) - (.25cm, 0)$) to[out=-90, in=20] ($(($(tokens.west) - (.25cm, 0)$) |- dual_policy.north)$);
        \coordinate (intermediate) at ($(tokens.west) + (-0.25cm, 0)$);
        % \coordinate (intermediate1) at (intermediate |- dual_policy.north);
        \draw[arrow] (g.south) 
        to[in=90, out=-90] (intermediate) 
        to[out=-90, in=90] (intermediate |- dual_policy.north);

        \draw[arrow, thick] (sk) -- (token_left);
        \draw[arrow] (token_left) -- (yes);
        \draw[arrow] (token_left) -- (no);
        \draw[arrow, thin] (token_left) -- (subgoals);
        \draw[arrow, thin] (subgoals) -- (token_left);
        \draw[arrow] (yes) -- (subgoal);
        \draw[arrow] (no) -- (goal_policy);

        \draw[arrow, thick] (dual_policy) -- (action);

    \end{tikzpicture}
    \caption{Inference pipeline of QPHIL.}
    \label{fig:inf_pipeline}
\end{wrapfigure}

The state quantizer \(\phi: {\cal S} \to \Omega\), with \(\Omega \equiv  \inte{1}{k}\),   %$
is used to map raw states into a set of $k$ landmark indexes (or tokens), %, each associated to a continuous embedding defined in a learned code-book $z:[[1,k]] \rightarrow \mathbb{R}^d$. We denote as $z_{\omega}=z(\omega)$ the embedding associated with token $\omega$ in that code-book. % 
 which serve as the building blocks for our planning strategy. These discrete representations are then processed by the plan generator, which assembles them into a coherent sequence that outlines the overall trajectory to be followed in the environment to reach the  requested goal \(g\). Given %depending
 any history of tokens \((\omega_0,\cdots,\omega_s)_{s > 0}\) and a targeted goal \(g \in {\cal G}\), % to be reached for the task at end%that quantizer, 
%the $z:[[1,k]] \rightarrow \mathbb{R}^d$ 
the plan generator produces sequences of tokens \((\omega_{s+1},\cdots,\omega_{s+l})\) auto-regressively until \(\omega_{s+l}=\dot{\omega}\) (with \(\dot{\omega}\) an extra end of sequence token that stops the generation), following: $\pi^\text{plan}\left((\omega_{s+1},\cdots,\omega_{s+l})\ |\ \phi(g), (\omega_i)_{i=0}^{s}\right)=\prod_{t=1}^l \pi^\text{plan}\left(\omega_{s+t}\ |\ \phi(g), (\omega_i)_{i=0}^{s+l-1}\right)$.  %$ \times \pi^{plan}(\dot{\omega}|\phi(g), (\omega_i)_{i=0}^{s+l})$, with $\dot{\omega}$ an extra index corresponding to the end of sequence token that stops generation.
It is used from the start token \(\omega_0=\phi(s_0)\) of the episode,  to propose a sequence of landmarks to follow using \(\pi^\text{landmark}: {\cal A} \times {\cal S} \times \Omega \to [0,1]\), before navigating through the final goal \(g\) using \(\pi^\text{goal}: {\cal A} \times {\cal S} \times {\cal G} \to [0,1]\). Optionally, it can also be used to re-plan after a given condition is reached (e.g. every \(n\) steps or when the agent leaves its current area), which is mostly useful for complex environments with stochasticity.    

\Cref{alg:qphil_inference} presents the inference pseudo-code of our QPHIL approach. For a given goal \(g\) and a start state \(s_0\), the process first samples a new plan, which corresponds to a sequence of landmarks to be reached sequentially before driving towards \(g\).  Then, until the first subgoal \(\omega\) of this sequence is reached (which happens when \(\phi(s)=\omega\)), \(\pi^\text{landmark}\) is used conditioned on the current state and the sub-goal \(\omega\) to sample actions to emit in the environment. When the sub-goal is reached, it is removed from the list, and we move to the next one, and so on until the list of sub-goals is empty. At that point, we should be ready to apply \(\pi^\text{goal}\) to move on toward the requested goal \(g\). A graphical representation of the inference pipeline is available in~\Cref{fig:inf_pipeline}. % and the pseudo-code in~\Cref{alg:qphil}. 


%of  discrete representations, referred to as tokens or landmarks, which serve as the building blocks for planning. These discrete representations are then processed by the sequence generator, which assembles them into a coherent sequence that outlines the overall trajectory to be followed. A graphical representation of the inference pipeline is available in~\Cref{fig:inf_pipeline} and the pseudo-code in~\Cref{alg:qphil}.

%To execute the plan, QPHIL uses two policies. The first policy navigates between these discrete representations, effectively moving from one identified landmark to the next in the sequence. After the sequence has been executed, a second policy is used to reach the goal within the last landmark.

\begin{algorithm}[H]
    \caption{\label{alg:qphil_inference}  Navigation with QPHIL}
    \begin{algorithmic}
    
    
    \Require Goal state \(g\), Start state \(s_0\), State quantizer \(\phi\), Sequence generator \(\pi^{plan}\), Navigation policies \(\pi^{\text{landmark}}\) and \(\pi^{\text{goal}}\)
    %\Ensure Action \(a\) to reach \(g\) from \(s\)
    \State \(\tau^< = (\phi(s_0))\); \(\tau^>=\{\}\);   \(s=s_0\); 
    \While{Not exceeding a  max number of steps} %$g$ is not reached (and not exceeding a  max number of steps)}
    \If{First step (or if re-planning is required)}% $\qquad$ \textit{   // Generate  future landmarks }
    \Comment{Generate  future landmarks}
        %\State 
        \State \(\tau^> \gets  (\omega_{1},\omega_{2},\dots, \dot{\omega}) \sim \pi^\text{plan}(.\ |\ \phi(g), \tau^<)\) %\mathcal{L} \gets G_{\text{seq}}(z_0, z_G)\)
    \EndIf
    
    %\If{\(\tau^>\) is not empty}
    \If{$\tau^>_0 \ != \ \dot{\omega}$}
        \(a \sim \pi^{\text{landmark}}(.\ |\ s, \tau^>_0)\)
    \Else\  \(a \sim \pi^{\text{goal}}(.\ |\ s, g)\)
    \EndIf
    \State Emit \(a\) in the environment and observe new state \(s'\)
    \State \(s \gets s'\); 
    %\If{\(\tau^>\) is not empty}
    \If{$\tau^>_0 \ != \ \dot{\omega}$}  
        \If{\(\phi(s)==\tau^>_0\)} %$\qquad \qquad \qquad \qquad$ \textit{   // Subgoal  reached, go to the next one}
        \Comment{Subgoal  reached, go to the next one}
        \State $\tau^<.\text{append}(\tau^>.\text{pop}(0))$; 
        \EndIf
    \Else\  
        \If{\(s\) is in \(g\)}  %$\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad$ \textit{    // Final goal  reached}
        \Comment{Final goal  reached}
            \State return;     
        \EndIf
    \EndIf
    
    
    
    \EndWhile
    %\Return \(a\)
    \end{algorithmic}
\end{algorithm}

% \input{inference_pipeline}

%This method is hierarchical. The sequence generator is effectively the high level policy and the two navigation policies are the low level policies. Unlike most hierarchical methods that invoke the high-level policy at each step, QPHIL generates the entire plan in a single step, creating a coherent sequence of landmarks that effectively guides the agent towards its goal.



The remainder of this section presents our learning methodology for every component of our QPHIL approach. 

\subsection{Tokenization}

\begin{wrapfigure}[17]{r}{.4\textwidth}
    \centering
        \vspace{-.73cm}
        \includegraphics[width=.4\textwidth]
        {figures/background_tokens_utra.pickle}
        \vspace{-.6cm}
        
        % \caption{Antmaze Ultra}
        \label{fig:tokenization-exemple_tokenization_exemple}
    \caption{Tokenization example. Each token has an associated color. The color of each point in the background correspond to the color of the associated token. It is noticeable that the tokens align with the walls thanks to the contrastive loss.}
\end{wrapfigure}

Discrete state tokens are learnt using a Vector Quantized-Variational AutoEncoder (VQ-VAE)~\cite{oord2018neural}, \textit{i.e.} an autoencoder with a finite latent space.
%A VQ-VAE is an autoencoder with a finite latent space, meaning that when a deterministic decoder is used, the output space also remains finite. This results in a well-defined set of tokens, where the VQ-VAE effectively maps states to their corresponding tokens.\\
% We considered several alternatives for tokenization, including DINO~\cite{caron2021emerging}, encoding the space to a sphere followed by K-means clustering, and manual segmentation using either a uniform grid or quantiles, as seen in Trajectory Transformer~\cite{janner2021offline}. However, we chose to use VQ-VAE for its simplicity and its ability to learn meaningful representations that we believe could generalize better. The implementation was straightforward, and initial results were promising, which reinforced our decision to keep this method.\\
The use of VQ-VAE for tokenization has been proposed in various domains, including time series analysis~\cite{lee2024leveraging}, video pretraining~\cite{tan2021vimpac}, and vision transformers~\cite{dong2023peco}; it has also been explored in offline reinforcement learning~\cite{jiang2022efficient, sudhakaran2023skill}. However, to the best of our knowledge, this type of tokenization has not been previously applied in planning.

% In simpler scenarios, this tokenization step could be replaced by a more straightforward, scripted approach (e.g., a grid for navigation). Nonetheless, our proposed method offers an automated solution that is particularly useful in cases where tokenization is not intuitive or where the state space is too large and complex.\\
% \input{figures/tokenization_exemple}


As defined in previous section, the state quantizer \(\phi\) %: {\cal S} \to \Omega\), with \(\Omega \equiv  \inte{1}{k}\),   %$
is used to map raw states into a set of $k$ tokens. It is composed of a state encoder $g: {\cal S} \rightarrow \mathbb{R}^d$, which maps the state space to a latent space of dimension $d$, and a learned code-book $z:\Omega  \rightarrow \mathbb{R}^d$, which  associates each token to a continuous embedding. %We denote as $z_{\omega}=z(\omega)$ the embedding associated with token $\omega$ in that code-book. % 
% which serve as the building blocks for our planning strategy.
From these, $\phi$ is defined as: $\phi(s)=\arg\min_{\omega \in \Omega} \Delta(g(s),z(\omega))$, with $\Delta$ the euclidean distance in the latent space.   


%The tokenizer is composed of three main elements: an encoder $g: {\cal S} \rightarrow \mathbb{R}^d$, a  \(\phi: {\cal S} \to \Omega\), with \(\Omega \equiv  \inte{1}{k}\), and a decoder $f: \mathbb{R}^d \rightarrow {\cal S}$. The encoder maps the state space to a latent space, the quantizer maps the latent space to a finite set of tokens, and the decoder maps the tokens back to the state space. 
As depicted in Figure~\Cref{fig:tokenization-pipeline}, three losses are considered to train these components. First, the VQ-VAE learns a meaningful representation by considering a reconstruction loss, which ensures that states can be decoded from tokens they are projected into:  % It ensures that tokens encode can be decoded to input states that are the input state can be decoded from the model gets close to the identity function, despite the finite output space:
\[
    \mathcal L_\text{recon} = \mathbb E_{s \sim \mathcal D}||f(z(\phi(s))) - s||_2^2,
\] where \(\mathcal D\) is the dataset and \(f: \mathbb{R}^d \rightarrow {\cal S}\) is a decoder network trained together with the code-book of token embeddings. 

As the gradient flow stops in the previous loss due to the discrete projection performed by $\phi$, we need to consider an additional commitment loss to learn the encoder parameters: 
\[
    \mathcal L_\text{commit} = \mathbb E_{s \sim \mathcal D}||g(s) - \text{sg}(z(\phi(s))||_2^2 + \beta||\text{sg}(g(s)) - z(\phi(s))||_2^2,
\]
where sg is the stop-gradient operator. The first term of this loss aims at attracting %latent encodings of states getting closer 
encoder  outputs close to the  code of the token states project into. %The second term, weighted by a hyperparameter \(\beta\), aims % is , \(\mathcal D\) is the dataset, \(g\) is the generator and \(q\) is the quantizer.
%
%that  
%
As explained by authors of the VQ-VAE architecture~\citep{van2017neural}, the embedding space grows arbitrarily if the token embedding does not train as fast as the encoder parameters. The second term, weighted by a hyperparameter \(\beta\), aims to prevent this issue. 

%A reconstruction loss is typically used to train a VQ-VAE. However, i
%In the context of offline reinforcement learning, this loss alone is insufficient to achieve meaningful tokenization. The reason is that two states can be numerically close but very different in their meaning in terms of RL. For instance, two positions on either side of a wall might be numerically close in a model that is map-agnostic, yet they represent entirely different scenarios in terms of trajectory planning.% This issue becomes particularly problematic in HIQL when the walls are thin, which is precisely the challenge our proposed method aims to address.

%\input{figures/thin_walls}

To introduce dynamics of the environment in the representation learned, we consider a third contrastive loss 
%
%
%In offline reinforcement learning, temporal proximity is more important than spatial proximity. Therefore, it has been proposed to use a contrastive loss
that incentivize temporally close states to be  assigned the same tokens, while temporally distant states receive different tokens. To achieve this, we use the triplet margin loss~\citep{balntas2016learning} applied to our setting:
\[
    \mathcal L_\text{contrastive} = \mathbb E_{\substack{s_t \sim \mathcal D\\ k \sim \inte {-\gamma} {\gamma} \\ k' \sim \Z \backslash \inte {-\gamma} {\gamma} }} \max\left\{\Delta(g(s_{t}), g(s_{t + k})) - d(g(s_{t}), g(s_{t + k'})), 0 \right\}, 
\]
where %\(\mathcal D\) is the dataset, \(g\) is the encoder, \(d\) is the Euclidean norm and \
\(\gamma\) is the time window used to specify temporal closeness of states in demonstration trajectories. %define what is a close state.
This loss is for instance of crucial importance in navigation settings with thin walls, where two states can be close in the input space, while corresponding to very different situations. 

The tokenizer loss, used in training is then a linear combination of the three previous losses:
\[
    \mathcal L_\text{tokenizer} = \mathcal L_\text{recon} + \alpha_1 \mathcal L_\text{commit} + \alpha_2 \mathcal L_\text{contrastive}.
\]

%An illustration of the training process is available in~\Cref{fig:tokenization-pipeline} and some examples of tokenization are shown in~\Cref{fig:tokenization-exemple}.
%This result correspond well to what we would have designed ourselves.
%Clusters (zone associated to a given token) are smaller where data is abundant and larger where data is scarce. Trajectories of the dataset are somehow visible in the shapes of the clusters. 


%The utility of the contrastive loss is perceivable in~\Cref{fig:tokenization-exemple_tokenization_exemple}. However, its strength is really revealed in~\Cref{fig:godot_tokenization_exemple}: walls are extremely thin and the tokenization completely take it into consideration. Clusters do not align perfectly with the walls, which we attribute to the scarcity of data near the wall.



\subsection{Sequence generation}

Once the tokenizer has been trained, states from dataset trajectories can be converted into sequences of discrete tokens. %, effectively transforming continuous state trajectories into symbolic sequences. The temporal contrastive loss used during training ensures consistency within these sequences, as depicted in~\Cref{fig:tokenization-pipeline}. This 
Temporal consistency induces sub-sequences of repeated tokens corresponding to positions  %manifests as repeated tokens for similar states 
within a given region. 
By applying a simple post-processing step $\eta^\phi(\tau)$ that removes consecutive repetitions of tokens in a trajectory $\tau$, we obtain  more concise sequences that succinctly represent key zones to traverse in the correct order. 
For instance, a tokenized sequence such as ``1 1 1 2 2 3 3 3 4 4'' is simplified to ``1 2 3 4'', reflecting the core structure of the trajectory. This process is illustrated in~\Cref{fig:compression}.

%A new dataset \(\mathcal S\) of simplified sequences of tokens is then generated and used to train the sequence generator. Additional cleaning steps are described in~\Cref{subsection:data-cleaning}.



%This dataset is used to train an encoder-decoder transformer model~\citep{vaswani2017attention}, which is a sequence-to-sequence model that is particularly well-suited for this task. The transformer is trained to predict the next token in the sequence given the previous tokens using the teacher forcing algorithm: at train time, given a sequence \((x_i)_{i < n}\) from the dataset, the model receives \(\left\{(x_i)_{i < m}\right\}_{m < n - 1}\). For each of these \(n\) beginning of sequence, the model generates a probability \((y_{i,j})_{j}\) for each token \(j\), where \(i\) is the index of the predicted element in the sequence. Output of the model is a probability distribution over tokens and we use the cross-entropy loss, which measures the difference between the predicted token probabilities and the actual tokens in the sequence:
Then, the planner $\pi^\text{plan}$ is trained following a teacher forcing approach on trajectories from ${\cal D}$, considering any future token of $\tau \in {\cal D}$ as the associated training goal: 
\[
    \mathcal{L}_\text{plan} = - \mathbb{E}_{\tau \sim {\cal D}} \quad \mathbb{E}_{\hspace{-0.5cm}\substack{t<|\tau|,\\\phi(\tau_t) \neq \phi(\tau_{t+1})}} % (\omega,\omega'), \\ \exists t \phi(\tau_t)=\omega \\ \wedge 
 %\phi(\tau_{t+1})=\omega'}}
 \ \  \mathbb{E}_{\hspace{-0.2cm}\substack{g \in {\cal G}, \\ \phi(g) \in \eta^\phi{\tau_{>t}}}} 
 \log \pi^\text{plan}(\phi(\tau_{t+1})\ |\ \phi(g),\eta^\phi(\tau_{\leq t})) ,
\]
with %${\cal D}$ a dataset of state trajectories associated with goals $g \in {\cal G}$,
\(|\tau|\) the number of states in \(\tau\), \(\tau_t\) the \(t\)-th state in \(\tau\), and \(\tau_{\leq t}\) (resp. \(\tau_{> t}\)) the history (resp.future) of \(\tau\) at step \(t\). 
%As any future state from any $s \in \tau$ can be consider as a    
We implement \(\pi^{plan}\) using a %n encoder-decoder 
transformer architecture~\citep{vaswani2017attention} \(h_\theta\), where \(\pi^\text{plan}(.\ |\ \phi(g),\eta^\phi(\tau_{\leq t}))\) is defined for any \(\omega \in \Omega\) using a softmax on the outputs of \(h_\theta(\phi(g),\eta^\phi(\tau_{\leq t}))\). 
While an alternative would be to consider a markov assumption stating that \(\pi^\text{plan}(.\ |\ \phi(g),\eta^\phi(\tau_{\leq t})) \approx \pi^\text{plan}(.\ |\ \phi(g), \phi(s_t)) \), we claim that dependency on the full history of the sequence is useful to anticipate the next token to be reached, as it can be leveraged to deduce the precise location of the agent in large landmark areas (which unknown during plan generation). %some knowledge about the precise location 

We note that this behavioral cloning way for training the planner could be complemented by an offline RL finetuning, following a goal-conditionned IQL algorithm for instance. Rather, we propose to consider in our experiments a data augmentation process on top of our behavioral cloning approach, which allowed us to obtain similar results, with greatly lower computational cost. Our data augmentation process relies on the opportunity of accurate trajectory stiching that our quantized space offers. %tokenized 
%Working with raw trajectories with continuous states limits the ability to mix history and future of different trajectories during training: from what distance of states could we consider that situations are enough similar to envision   
Assuming that it is easy for our low-level policy $\pi^\text{landmark}$ to reach, from any state $s \in {\cal S}$, any state $s'$ such that $\phi(s')=\phi(s)$, we propose to augment ${\cal D}$ with all possible mix of trajectories that pass through the same landmark and own a similar future quantized state: $\forall (\tau,\tau') \in {\cal D}^2, t \in [[0,|\tau|]], t' \in [[0,|\tau'|]], l \in [[t+1,|\tau|]], l' \in [[t'+1,|\tau'|]]: \phi(s_t)=\phi(s'_{t'}) \wedge \phi(s_l)=\phi(s'_{l'})  \implies ((s_i)_{i=0}^{t},(s'_i)_{i=t'+1}^{l'}) \in {\cal D} \wedge ((s'_i)_{i=0}^{t'},(s_i)_{i=t+1}^{l}) \in {\cal D} $.  %$ trajectories$ from any state $s$ 
%
%
%We propose to use a simple data augmentation technique: for each pair of sequence, if the final token of the first sequence is in the second one, we add a new trajectory in the dataset: the first sequence followed by the end of the second one.
%We could generate a lot more data by considering all tokens from the first sequence instead. However, using only the last one generate enough new data to be useful and is much faster. 
%It also helps to keep a balance between the number of real sequences and generated ones.
This technique is illustrated in~\Cref{fig:data_augmentation}. %We leave the design and analysis of more complex stitching mechanisms for future work. 
% While we create many more sequences\footnote{The dataset size can be multiplied by a factor of 10.}, it can easily be implemented in a data efficient way. The pair of sequences and stitching index are stores and concatenation is done on the fly. This could allow more data generation by considering more than the last index of the first sequence or by successively stitching sequences from stitched sequences.


%\[
%    \mathcal{L}_\text{transformer} = - \sum_{i=0}^{n-1} \log\dfrac{\exp x_{t, a_i}}{\sum_m \exp x_{i, m}}  ,
%\]
%where \(a_i\) is the actual token index for the element \(i\) of the sequence and for all \(j\), \(y_{i, j}\) is the predicted probability of the token \(m\) for the element \(i\).

%In order to generate sequences that start from the initial position and end at the goal, the encoder of the transformer receives the goal token, a start of sequence token and then the initial token. 

%During inference, the encoder is fed the input sequence. Then, until the model outputs the end of sequence token, the output of the encoder and previously generated tokens (none at the first step) are fed to the decoder. A softmax layer and a temperature parameter \(T\) are then used on the output of the decoder to create a distribution over the tokens. The token is then sampled from this distribution:
%\[
%    y_t \sim \text{Cat}\left(\dfrac{\exp\left(\dfrac{z^i_t}{T}\right)}{\sum_{j}\exp\left(\dfrac{z^j_{t}}{T}\right)} \right)_i,
%\] 
%where \(z_t\) is the output of the decoder at step \(t\). This process is repeated until the model outputs the end of sequence token. Pseudo-code of the inference is available in~\Cref{alg:inference_transformer}.

% \input{sequence_generation}


\subsection{Low-level policies}

%The final component of our algorithm is the policy that learns action execution. This policy approximates the distribution \(\pi(a | s, g)\), where \(a\) is an action form that dataset associated with a state \(s\) and either a goal or a subgoal \(g\). Initially, we attempted to develop a single unified policy for both goals and subgoals. However, this approach underperformed, leading us to adopt two separate policies. The first, the ``goal policy'' takes the current state and goal as input and outputs a distribution of actions, trained using the standard IQL algorithm. The second, the ``subgoal policy'' is a variant of IQL adapted for subgoal-directed tasks.

As described above, two low-level policies \(\pi^\text{landmark}\) and \(\pi^\text{goal}\) have to be trained to perform actions in the environment. Both of these politics are trained via IQL, whose principle is described in section \ref{preliminaries}. As \(\pi^\text{goal}\) works with initial (non tokenized) goals to allow final precise navigation in the final area of the task, we consider a classical $V$ network $V^\text{goal}$ trained using \eqref{iqlv} on raw states and goals, independently from all other components, from which the policy is extracted using AWR: 
\begin{align}
    \label{pigoal}
    \mathcal{L}_{\pi^{\text{goal}}} & = \mathbb{E}_{(s_t,s_{t+1},g)\sim{\cal D}}[\exp (\beta \cdot (V^{\text{goal}}(s_{t+1},g) - V_{\theta_V}(s_t,g))) \log \pi^{\text{goal}}(s_{t+1}|s_t,g)] %\\
    %\mathcal{L}_{\pi^l}(\theta_l) & = \mathbb{E}_{(s_t,a_t,s_{t+1},s_{t+k})}[\exp(\beta \cdot (V_{\theta_V}(s_{t+1},s_{t+k}) - V_{\theta_V}(s_t,s_{t+k})) \log \pi_{\theta_l}^l(a_t|s_t,s_{t+k})]
\end{align}

Our policy \(\pi^\text{landmark}\) uses the same principle, but replaces  the distant goal $g$ by sub-goals defined as the next landmark to be reached from quantized trajectories in the buffer of training transitions. That is, given any training trajectory $\tau=((s_t,a_t,s_{t+1},g))_{t=0}^{|\tau|-1}$, we consider a sequence of relabelled transitions $\tilde{\tau}=((s_t,a_t,s_{t+1},next(\tau,t))_{t=0}^{|\tau|-1}$, where $next(\tau,t)= \phi\left(s_{\min(\{t \in [[t+1,|\tau|]]: %\substack{l>t, \\ 
\phi(s_l)\neq \phi(s_t)\})}\right)$ corresponds to the next different subgoal in the sequence of quantized states  $(\phi(s_t))_{t=0}^{|\tau|-1}$ of the trajectory $\tau$. $V^\text{landmark}$ is then trained on that set of relabelled transitions $\tilde{\cal D}$. Then, the policy is extracted similarly as for $\pi^\text{goal}$ using \eqref{pigoal} %on  AWR policy extraction is performed using \eqref{awr} 
on $\tilde{\cal D}$ rather than ${\cal D}$, in order to obtain $\pi^\text{landmark}$ via a relabelled IQL from $V^\text{landmark}$.  %filtering out every transition whose relabelled goal is $\dot{omega}$,    %  training transition $(s_t,a_t,s_{t+1},g)$ from trajectory $\tau$ is relabelled with  \((s_t,a_t,s_{t+1} %using the quantizer from the rather than  

%Although it might seem intuitive to train the subgoal policy using IQL with a token representation of the goal, this introduces unnecessary complexity without providing significant benefits. At inference time, the subgoal policy has to the next subgoal, which corresponds to a neighboring token. Training the policy to reach long-term goals would undermine the planner, wasting resources and potentially degrading performance. Instead, during training, the goal provided to the subgoal policy is the next token in the episode’s token sequence, aligning with the inference process.

%While both HIQL and QPHIL are hierarchical extensions of IQL, their high-level policies differ significantly. HIQL uses the same value function for both its high and low-level policies. Although using a shared value function for our two policies would have been more elegant, the disparity in goal representations made it impractical.



%\subsubsection{Data augmentation}\label{sec:data-augmentation}


%One of the most crucial aspects of offline reinforcement learning is stitching. Incorporating it in the training part is not easy for most algorithms when the data is continuous as one exact state is unlikely to be repeated. However, in our case, we have a discrete representation of the state space, which means that states (here tokens) are repeated often. This allows us to use data augmentation techniques that are not possible in continuous spaces.









==> sections/pipeline_alexi.tex <==

\begin{wrapfigure}{l}{.4\textwidth}
    \centering
    \begin{tikzpicture}[
    node distance=.3cm, 
    every node/.style={fill=white, font=\scriptsize}, 
    encoder/.style={trapezium, trapezium angle=70, draw=yellow!70!black, minimum width=1cm, minimum height=.75cm, rounded corners=.5pt, thick, fill=yellow!10},
    decoder/.style={trapezium, trapezium angle=110, draw=yellow!70!black, minimum width=1 cm, minimum height=.75cm, rounded corners=.5pt, thick, fill=yellow!10},
    latent/.style={rectangle, draw, rounded corners=.5pt, thick},
    loss/.style={rectangle, draw, rounded corners=2.5pt, draw=cyan!70!black, thick, fill=cyan!10},
    rect/.style={rectangle, draw, rounded corners=2.5pt, thick},
    codebook/.style={matrix of nodes, nodes={draw, rectangle, minimum width=0.25cm, minimum height=0.5cm, anchor=center}, rounded corners=.5pt, thick},
    arrow/.style={-Stealth}
]
    \node[fill=none] (s0) {\(s_0\)};
    \node[fill=none, left=of s0] (g) {\(g\)};
    \begin{scope}[on background layer]
        \node[fit=(g.north west) (s0.south east), fill=gray!10, draw=gray!70!black, thick, rounded corners=2.5pt] (rectangle) (input) {};
    \end{scope}

    \node[rect, below=of input] (tokenizer) {Tokenizer};

    \node[rect, below=1cm of tokenizer] (transformer) {Transformer};

    \coordinate (midpoint) at ($(tokenizer)!0.5!(transformer)$);
    \node[fill=none] at ($(midpoint) + (.75,0)$) (token_s0) {\(\phi(s_0)\)};
    \node[fill=none] at ($(midpoint) - (.75,0)$) (token_g) {\(\phi(g)\)};
    \begin{scope}[on background layer]
        \node[fit=(token_g.north west) (token_s0.south east), fill=purple!10, draw=purple!70!black, thick, rounded corners=2.5pt] (rectangle) at (midpoint) (tokens) {};
    \end{scope}


    \node[rect, below=of transformer] (subgoals) {Subgoal sequence};
    % \node[fill=none, left=.5cm of subgoals] (token_left) {\footnotesize{Token left ?}};
    % \node[fill=none, below=of token_left] (no) {\footnotesize{No}};
    % \node[fill=none, right=of no] (yes) {\footnotesize{Yes}};
    

    % \node[rect, below=of subgoals, draw=purple!70!black, fill=gray!10] (subgoal) {Next token};

    % \node[rect, below=of subgoal, draw=cyan!70!black, fill=cyan!10] (subgoal_policy) {IQL Subgoal};
    % \node[rect, left=of subgoal_policy, below=of no, draw=cyan!70!black, fill=cyan!10] (goal_policy) {IQL};

    % \begin{scope}[on background layer]
    %     \node[fit=(subgoals.north east) ($(token_left.west |- goal_policy.south)$), fill=yellow!10, draw=yellow!70!black, thick, rounded corners=2.5pt] (rectangle) at ($(subgoals.east |- subgoal_policy.south)!.5!(token_left.north west)$) (dual_policy) {};
    % \end{scope}

    % \node[fill=none, below=of dual_policy] (action) {Action};


    \node[fill=none, right=of tokens] (sk) {\(s_k\)};
    \node[rect, below=of sk] (tokenizer1) {Tokenizer};
    \node[fill=none, below=of tokenizer1] (token_sk) {\(\phi(s_k)\)};
    \node[fill=none, below=of token_sk] (is_goal) {\(\omega = \phi(g)\) ?};
    \node[fill=none, below=.6cm of is_goal.east, fill=cyan!10, draw=cyan!70!black, thick, rounded corners=2.5pt] (pi_goal) {\(\pi^\textnormal{goal}(a\ |\ s_k, g)\)};


    \node[fill=none, left=of pi_goal] (is_subgoal) {\tiny is subgoal ?};
    \node[fill=none, below=.6cm of is_subgoal.west] (get_token) {\tiny Get next subgoal};
    \node[fill=none, below=.7cm of is_subgoal.east, xshift=1.cm, fill=cyan!10, draw=cyan!70!black, thick, rounded corners=2.5pt] (pi_subgoal) {\(\pi^\textnormal{landmark}(a\ |\ s_k, \omega\))};




    \draw[arrow] (input) -- (tokenizer);
    \draw[arrow] (sk.south) -- (tokenizer1.north);

    \draw[arrow] (tokenizer) -- (token_s0);
    \draw[arrow] (tokenizer) -- (token_g);
    \draw[arrow] (tokenizer1.south) -- (token_sk.north);
    \draw[arrow] (token_sk.south) -- (is_goal.north);
    \draw[arrow] ($(is_goal.south) + (.3, 0)$) -- (pi_goal.north) node[near start, right=.3cm, fill=none] {\tiny Yes};
    \draw[arrow] ($(is_goal.south) - (.3, 0)$) -- (is_subgoal.north) node[near start, left=.3cm, fill=none] {\tiny No};
    \draw[arrow] ($(is_subgoal.south) - (.3, 0)$) -- (get_token.north) node[near start, left=.1cm, fill=none] {\tiny No};
    \draw[arrow] ($(is_subgoal.south) + (.3, 0)$) -- ($(pi_subgoal.north) - (.3, 0)$) node[midway, right=.3cm, fill=none] {\tiny Yes};
    % \draw[arrow] (pi_goal) -- ($(env.north) - (.3, 0)$) node[midway, left, fill=none] {\(a\)};
    % \draw[arrow] ($(env.north) + (.3, 0)$) -- (pi_goal) node[midway, right, fill=none] {\(s_k\)};

    \draw[arrow] (token_s0) -- (transformer);
    \draw[arrow] (token_g) -- (transformer);

    \draw[arrow] (transformer) -- (subgoals);

    \node[fill=none, below=.3cm of subgoals, xshift=.5cm] (omega) {\(\omega\)};
    

    \draw[arrow] ($(get_token.north) - (.45, 0)$) to[in=-90, out=90] ($(get_token.north) - (.45, -.5)$) to[in=180, out=90] (is_goal.west);
    % \draw[arrow] (subgoals) -- ($(get_token.north) - (.55, 0)$);
    \draw[arrow] ($(get_token.north |- subgoals.south) - (.55, 0)$) -- ($(get_token.north) - (.55, 0)$);
    % \node[fill=none, at={}, xshift=-.55cm] (pi_subgoal) {\(\pi^\textnormal{landmark}(a\ |\ s_k, )\)};

    % \draw[arrow] ($(subgoals.south) - (.25cm, 0)$) -- ($(subgoal.north) - (.25cm, 0)$);
    % \draw[arrow] ($(subgoal.north) + (.25cm, 0)$) -- ($(subgoals.south) + (.25cm, 0)$);
    % \draw[arrow] (subgoal) -- (subgoal_policy);

    % % \draw[arrow] (g.south) to[in=90, out=-90] ($(tokens.west) - (.25cm, 0)$) to[out=-90, in=20] ($(($(tokens.west) - (.25cm, 0)$) |- dual_policy.north)$);
    % \coordinate (intermediate) at ($(tokens.west) + (-0.25cm, 0)$);
    % % \coordinate (intermediate1) at (intermediate |- dual_policy.north);
    % \draw[arrow] (g.south) 
    % to[in=90, out=-90] (intermediate) 
    % to[out=-90, in=90] (intermediate |- dual_policy.north);

    % \draw[arrow, thick] (sk) -- (tokenizer);
    % \draw[arrow] (token_left) -- (yes);
    % \draw[arrow] (token_left) -- (no);
    % \draw[arrow, thin] (token_left) -- (subgoals);
    % \draw[arrow, thin] (subgoals) -- (token_left);
    % \draw[arrow] (yes) -- (subgoal);
    % \draw[arrow] (no) -- (goal_policy);

    % \draw[arrow, thick] (dual_policy) -- (action);
    % \begin{scope}[on background layer]
    %     \node[fit=(subgoals.north east) ($(token_left.west |- goal_policy.south)$), fill=yellow!10, draw=yellow!70!black, thick, rounded corners=2.5pt] (rectangle) at ($(subgoals.east |- subgoal_policy.south)!.5!(token_left.north west)$) (dual_policy) {};
    % \end{scope}
    \coordinate (sw_corner) at ($(get_token.south west |- pi_subgoal.south) - (0,0)$);
        \begin{scope}[on background layer]
        \node[fit=(sw_corner) ($(pi_subgoal.east |- is_goal.north)$), fill=yellow!10, draw=yellow!70!black, thick, rounded corners=2.5pt] (rectangle) at ($(pi_subgoal.east |- is_goal.north)!.5!(get_token.south west |- pi_subgoal.south)$) (dual_policy) {};
    \end{scope}

    \node[fill=none, below=.5cm of dual_policy] (env) {Environment};
    \draw[arrow] ($(env.north |- dual_policy.south)$) -- ($(env.north)$) node[midway, left, fill=none] {\(a\)};
    \draw[arrow] ($(env.east)$) to[in=-90, out=0] ($(dual_policy.east) + (.2, -1.2)$) to[in=-90, out=90] ($(dual_policy.east) + (.2, 1.5)$) to[in=-0, out=90] (sk.east);

\end{tikzpicture}
    % \begin{tikzpicture}[
    %     node distance=.3cm, 
    %     every node/.style={fill=white, font=\scriptsize}, 
    %     encoder/.style={trapezium, trapezium angle=70, draw=yellow!70!black, minimum width=1cm, minimum height=.75cm, rounded corners=.5pt, thick, fill=yellow!10},
    %     decoder/.style={trapezium, trapezium angle=110, draw=yellow!70!black, minimum width=1 cm, minimum height=.75cm, rounded corners=.5pt, thick, fill=yellow!10},
    %     latent/.style={rectangle, draw, rounded corners=.5pt, thick},
    %     loss/.style={rectangle, draw, rounded corners=2.5pt, draw=cyan!70!black, thick, fill=cyan!10},
    %     rect/.style={rectangle, draw, rounded corners=2.5pt, thick},
    %     codebook/.style={matrix of nodes, nodes={draw, rectangle, minimum width=0.25cm, minimum height=0.5cm, anchor=center}, rounded corners=.5pt, thick},
    %     arrow/.style={-Stealth}
    % ]
    %     \node[fill=none] (s0) {\(s_0\)};
    %     \node[fill=none, left=of s0] (g) {\(g\)};
    %     \begin{scope}[on background layer]
    %         \node[fit=(g.north west) (s0.south east), fill=gray!10, draw=gray!70!black, thick, rounded corners=2.5pt] (rectangle) (input) {};
    %     \end{scope}

    %     \node[rect, below=.5cm of s0.south east] (tokenizer) {Tokenizer};

    %     \node[rect, below=1cm of tokenizer] (transformer) {Transformer};

    %     \coordinate (midpoint) at ($(tokenizer)!0.5!(transformer)$);
    %     \node[fill=none] at ($(midpoint) - (1,0)$) (token_s0) {Token \(s_0\)};
    %     \node[fill=none] at ($(midpoint) + (1,0)$) (token_g) {Token \(g\)};
    %     \begin{scope}[on background layer]
    %         \node[fit=(token_s0.north west) (token_g.south east), fill=purple!10, draw=purple!70!black, thick, rounded corners=2.5pt] (rectangle) at (midpoint) (tokens) {};
    %     \end{scope}

    %     \node[rect, below=of transformer] (subgoals) {Subgoal sequence};
    %     \node[fill=none, left=.5cm of subgoals] (token_left) {\footnotesize{Token left ?}};
    %     \node[fill=none, below=of token_left] (no) {\footnotesize{No}};
    %     \node[fill=none, right=of no] (yes) {\footnotesize{Yes}};
    %     \node[fill=none, above=of token_left] (sk) {\(s_k\)};

    %     \node[rect, below=of subgoals, draw=purple!70!black, fill=gray!10] (subgoal) {Next token};

    %     \node[rect, below=of subgoal, draw=cyan!70!black, fill=cyan!10] (subgoal_policy) {IQL Subgoal};
    %     \node[rect, left=of subgoal_policy, below=of no, draw=cyan!70!black, fill=cyan!10] (goal_policy) {IQL};

    %     \begin{scope}[on background layer]
    %         \node[fit=(subgoals.north east) ($(token_left.west |- goal_policy.south)$), fill=yellow!10, draw=yellow!70!black, thick, rounded corners=2.5pt] (rectangle) at ($(subgoals.east |- subgoal_policy.south)!.5!(token_left.north west)$) (dual_policy) {};
    %     \end{scope}

    %     \node[fill=none, below=of dual_policy] (action) {Action};


    %     \draw[arrow] (input) -- (tokenizer);

    %     \draw[arrow] (tokenizer) -- (token_s0);
    %     \draw[arrow] (tokenizer) -- (token_g);

    %     \draw[arrow] (token_s0) -- (transformer);
    %     \draw[arrow] (token_g) -- (transformer);

    %     \draw[arrow] (transformer) -- (subgoals);

    %     \draw[arrow] ($(subgoals.south) - (.25cm, 0)$) -- ($(subgoal.north) - (.25cm, 0)$);
    %     \draw[arrow] ($(subgoal.north) + (.25cm, 0)$) -- ($(subgoals.south) + (.25cm, 0)$);
    %     \draw[arrow] (subgoal) -- (subgoal_policy);

    %     % \draw[arrow] (g.south) to[in=90, out=-90] ($(tokens.west) - (.25cm, 0)$) to[out=-90, in=20] ($(($(tokens.west) - (.25cm, 0)$) |- dual_policy.north)$);
    %     \coordinate (intermediate) at ($(tokens.west) + (-0.25cm, 0)$);
    %     % \coordinate (intermediate1) at (intermediate |- dual_policy.north);
    %     \draw[arrow] (g.south) 
    %     to[in=90, out=-90] (intermediate) 
    %     to[out=-90, in=90] (intermediate |- dual_policy.north);

    %     \draw[arrow, thick] (sk) -- (token_left);
    %     \draw[arrow] (token_left) -- (yes);
    %     \draw[arrow] (token_left) -- (no);
    %     \draw[arrow, thin] (token_left) -- (subgoals);
    %     \draw[arrow, thin] (subgoals) -- (token_left);
    %     \draw[arrow] (yes) -- (subgoal);
    %     \draw[arrow] (no) -- (goal_policy);

    %     \draw[arrow, thick] (dual_policy) -- (action);

    % \end{tikzpicture}
    \caption{Inference pipeline of QPHIL.}
    \label{fig:inf_pipeline1}
\end{wrapfigure}

==> sections/preliminaries_3009_13h.tex <==
\label{preliminaries}
% Reinforcement Learning (RL) correspond to learning an agent (model) that will interact with an environment. An environment can be a video-game, a robot arm, \dots. Interaction with the environment occurs sequentially over discrete time steps. At each time step, the environment provides a state \(s \in \mathcal S\), which represents the current situation. The agent, governed by a policy \(\pi\) (a conditioned probability distribution over actions), selects an action \(a \in \mathcal{A}\) based on this state. In response, the environment returns a reward \(r \in \R\), a numerical value that quantifies the quality of the action in relation to the agent's objectives. The sequence of states, actions, and rewards observed over time is referred to as a trajectory \(\tau\). The primary objective is to maximize the cumulative reward \(J\) (also called return), which can be expressed as:
\textbf{Offline Goal Conditioned Reinforcement Learning} We place ourselves in the context of offline goal-conditioned Reinforcement Reinforcement Learning. Offline Goal-Conditioned Reinforcement Learning (offline GCRL) involves training an agent to interact with an environment to reach specifc goals. It is typically modeled as a Markov Decision Process (MDP) defined by a tuple \((\mathcal{S}, \mathcal{A}, p, \mu, r)\), a dataset of demonstration trajectories \(\mathcal{D}\) and a given goal space \(\mathcal{G}\), where \(\mathcal{S}\) is the state space, \(\mathcal{A}\) the action space, \(p(s_{t+1}|s_t, a_t) \in \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{P}(\mathcal{S})\) the transition dynamics, $\mu \in \mathcal{P}(\mathcal{S})$ the initial state distribution and \(r(s_t,g) \in \mathcal{S} \times \mathcal{G} \rightarrow \mathbb{R}\) the goal-conditioned reward function given the goal space \(\mathcal{G}\). % In this framework, the environment can represent diverse systems, such as video games or robotic arms, with episodic interactions occurring sequentially over discrete time steps. 
In GCRL, the reward is sparse as \(r(s,g) = 1\) only when \(s\) reached \(g\) and \(0\) otherwise. Hence, our objective is to leverage the dataset \(\mathcal{D}\) composed of reward-free pre-recorded trajectoires \(\tau = (s_0,a_0,...,s_{T-1},a_{T-1},s_T)\) to learn the policy \(\pi(a_t|s_t,g)\) to reach given goals \(g \in \mathcal{G}\) by maximizing the expected cumulative reward, or return, \(J(\pi)\), which can be expressed as: \(J(\pi) = \mathbb{E}_{\substack{g \sim d_g\\ \tau \sim d_\pi}} \left[ \sum_{t=0}^T \gamma^t r(s_t, g) \right]\)
where \(\gamma\) is a discount factor, \(d_g\) represents the goal distribution and \(d_\pi\) is the trajectory distribution. The trajectory distribution \(d_\pi(\tau, g)\) is defined by:
\(d_\pi(\tau, g) = \mu(s_0) \prod_{t=0}^T \pi(a_t|s_t, g)p(s_{t+1}|s_t,a_t)\) and represents the distribution of trajectory when the policy is used. %As we operate in the offline goal-conditioned RL setting, our goal is to learn 
% It is defined according to the probability of getting each trajectory according to the initial state distribution, the goal distribution, the policy and the environment response to actions.

\begin{comment}
\paragraph*{Implicit Q-Learning (IQL)}

Implicit \(Q\)-learning~\citep{kostrikov2021offline} is designed to overcome the shortcomings of \(Q\)-learning: learning a function \(\mathcal Q: \mathcal S \times \mathcal A \to \R\) that estimates the expected return of an action in a given state. A value function \(V\) is learnt to estimate how much a state if ``worth'':
\[
    V: s \mapsto \max_a \tilde Q(s,a),
\] where \(\tilde Q\) is the \(Q\)-function. This intermediary application limits errors created by ``lucky'' transitions. There is not easy access to \(\tilde Q\). Hence, a learnt \(Q\)-function \(Q\) will be used with the action from the expert (actions from the dataset) to approximate \(\max\tilde Q(s, \cdot)\) and both functions will be trained at the same time. The value function is trained with a target network with \textsc{Polyak} averaging. This value function is trained using the following loss
\begin{equation}
\label{iqlv}
    \mathcal L_V = \mathbb E_{(s, a) \sim \mathcal D} \left[ L_2^\tau \left( Q(s, a) - V(s)\right) \right],
\end{equation}
where \(L_2^\tau : u \mapsto |\tau - \mathbbm{1}_{\R_-^\star} |u^2\) is the expectile loss. The \(Q\)-function is then updated using the value function with a MSE loss
\[
    \mathcal L_Q = \mathbb E_{(s, a, s') \sim \mathcal D} \left[ \left( r(s,a) + \gamma V(s') - Q(s,a) \right)^2\right].
\]

Those functions are then finally used to extract a policy. To prevent the use of out-of-samples actions, they use Advantage Weighted Regression (AWR)~\cite{peters2007reinforcement, wang2018exponentially, peng2019advantage, nair2020awac}:
\begin{equation}
\label{awr}
    \mathcal L_\pi = -\mathbb E_{(s,a) \sim \mathcal D} \left[ \exp\left(\beta(Q(s,a) - V(s)\right)\log \pi(a|s) \right],
\end{equation}
where \(\beta \in (0, +\infty]\) is an inverse temperature and \(\pi\) is the policy. This loss correspond to a variant of simple behavior cloning: the \(\log\)likelihood is used. However, this loss is weighted by the exponential term. This term is close to zero when the value of the state is higher than the value of the expert's action according to the \(Q\)-function, and high when the action as a high value when compared to the value function. This gives less weight in the loss to actions that where not optimal. 
\end{comment}

\begin{comment}
\paragraph*{Implicit Q-Learning (IQL)}
The main issue of offline RL is the overestimation of the value of out-of-distribution actions when minimizing the temporal difference error leading the policy to favor overestimated actions:
\begin{equation}
    \label{td_loss}
    \mathcal{L}_{TD} = \mathbb{E}_{(s_t,a_t,s_{t+1}) \sim \mathcal{D}} \left [  (r(s_t,a_t) + \gamma \; \underset{a_{t+1}}{\max} \; Q_{\hat{\theta}_Q}(s_{t+1},a_{t+1})-Q_{\theta_Q}(s_t,a_t))^2 \right ]
\end{equation}
with \(r(s_t,a_t)\) the task reward, \(\hat{\theta}_Q\) the parameters of a target network. Without further interactions with the environment, those overestimations cannot be corrected. While other work propose to regularize the loss function to avoid sampling out-of-distribution actions, \cite{kostrikov2021offline} proposes IQL which estimates the in-distribtion \(\max Q\) operator with expectile regression. To do so, it learns a state value function \(V_{{\theta}_V}(s_t)\) along a state-action value function \(Q_{{\theta}_{Q}}(s_t,a_t)\):
\begin{align}
    \label{iql_losses}
    \mathcal{L}_V(\theta_V) & = \mathbb{E}_{(s_t,a_t) \sim \mathcal{D}} \left [ L_2^\tau(Q_{\hat{\theta}_Q}(s_t,a_t) - V_{\theta_V}(s_t)) \right ] \\
    \mathcal{L}_Q(\theta_Q) & = \mathbb{E}_{(s_t,a_t,s_{t+1}) \sim \mathcal{D}} [ r(s_t,a_t) + \gamma \; V_{\theta_V}(s_{t+1})-Q_{\theta_Q}(s_t,a_t))^2 ]
\end{align}
with \(L_2^\tau(u) = |\tau - \mathbbm{1}(u < 0)|u^2, \tau \in [0.5,1)\) the expectile loss, which corresponds to an asymmetric square loss which penalises positive values more than negative ones the more \(\tau\) tends to \(1\), consequently leading \(V_{\theta_V}(s_t)\) to lean towards \( \max_{\; a_{t+1} \in \mathcal{A}, \text{ st. } \pi_\beta(a_{t}|s_t) > 0} \; Q_{\hat{\theta}_Q}(s_t,a_t)\) with \(\pi_\beta\) the datasets behavior policy.
The use of two different networks is justified to train the value function only on the dataset action distribution without incorporating environment dynamics in the TD-error loss, which avoids the overestimation induced by lucky transitions. Then, the trained \(V_{{\theta}_V}(s_t)\) and \(Q_{{\theta}_{Q}}(s_t,a_t)\) are used to compute advantages to extract a policy \(\pi_{\theta_\pi}\) with advantage weighted regression (AWR):
\begin{equation}
\label{awr_loss}
    \mathcal L_\pi(\theta_\pi) = -\mathbb E_{(s_t,a_t) \sim \mathcal D} \left[ \exp\left(\beta(Q_{\hat{\theta}_Q}(s_t,a_t) - V_{\theta_V}(s_t)\right)\log \pi_{\theta_\pi}(a_t|s_t) \right],
\end{equation}
with  \(\beta \in (0, +\infty]\) an inverse temperature. This correspond to the cloning of the demonstrations with a biais towards actions that present a higher Q-value.
\end{comment}

\begin{comment}
\paragraph*{Hierarchical Implicit Q-Learning (HIQL)}
In the offline GCRL setting, the rewards are sparse, only giving signals for states where the goal is reached. Hence, as bad actions can be corrected by good actions and good actions can be polluted by bad actions in the future of the trajectory, offline RL methods are at risk of wrongly label bad actions as good one, and conversely good actions as bad ones. This leads to the learning of a noisy goal-condidtioned value function: \(\hat{V}(s_t,g) = V^*(s_t,g) + N(s_t,g)\) where \(V^*\) corresponds to the optimal value function and \(N\) corresponds to a noise. As the 'signal-to-noise' ratio worsens for longer term goals, offline RL methods such as IQL struggle when the scale of the GCRL problem increases, leading to noisy advantages in IQL's AWR weights for which the noise overtakes the signal. To alleviate this issue, HIQL proposes to learn a noisy goal conditioned action-free value function as in IQL: 
\begin{equation}
    \label{iqlv}
    \mathcal{L}_V(\theta_V) = \mathbb{E}_{(s_t,s_{t+1}) \sim \mathcal{D}, g \sim p(g|\tau)} \left [ L_2^\tau(r(s_t,g) + \gamma V_{\hat{\theta}_V}(s_{t+1},g) - V_{\theta_V}(s_t,g)) \right ]
\end{equation}
and to use it to learn two policies \(\pi^h(s_{t+k}|s_t,g)\) to generate subgoals from the goal and \(\pi^l(a_t|s_t,g)\) to generate actions to reach the subgoals:
\begin{align}
    \label{iql_losses}
    \mathcal{L}_{\pi^h}(\theta_h) & = \mathbb{E}_{(s_t,s_{t+k},g)}[\exp (\beta \cdot (V_{\theta_V}(s_{t+k},g) - V_{\theta_V}(s_t,g))) \log \pi_{\theta_h}^h(s_{t+k}|s_t,g)] \\
    \mathcal{L}_{\pi^l}(\theta_l) & = \mathbb{E}_{(s_t,a_t,s_{t+1},s_{t+k})}[\exp(\beta \cdot (V_{\theta_V}(s_{t+1},s_{t+k}) - V_{\theta_V}(s_t,s_{t+k})) \log \pi_{\theta_l}^l(a_t|s_t,s_{t+k})]
\end{align}
With this division, each policy profits from higher signal-to-noise ratios as the low-policy only queries the value function for nearby subgoals \(V(s_{t+1},s_{t+k})\) and the high policy queries the value function for more diverse states leading to dissimilar values \(V(s_{t+k},g)\).
\end{comment}

\paragraph*{Hierarchical Implicit Q-Learning (HIQL)}
\begin{comment}
The main issue of offline RL is the overestimation of the value of out-of-distribution actions when minimizing the temporal difference $Q$ values with classical  (state,action)-value networks. % leading the policy to favor overestimated actions:
%\begin{equation}
%    \label{td_loss}
%    \mathcal{L}_{TD} = \mathbb{E}_{(s_t,a_t,s_{t+1}) \sim \mathcal{D}} \left [  (r(s_t,a_t) + \gamma \; \underset{a_{t+1}}{\max} \; Q_{\hat{\theta}_Q}(s_{t+1},a_{t+1})-Q_{\theta_Q}(s_t,a_t))^2 \right ]
%\end{equation}
%with \(r(s_t,a_t)\) the task reward, \(\hat{\theta}_Q\) the parameters of a target network. 
Without further interactions with the environment, those over-estimations cannot be corrected. While other work propose to regularize the loss function to avoid sampling out-of-distribution actions, \cite{kostrikov2021offline} proposes IQL, which estimates the in-distribution \(\max Q\) operator via a value function \(V_{{\theta}_V}\) with expectile regression, using  %To do so, it learns a state value function \(V_{{\theta}_V}(s_t)\):  %along a state-action value function \(Q_{{\theta}_{Q}}(s_t,a_t)\):
%\begin{align}
%    \label{iql_losses}
   % \mathcal{L}_V(\theta_V) & = \mathbb{E}_{(s_t,a_t) \sim \mathcal{D}} \left [ L_2^\tau(Q_{\hat{\theta}_Q}(s_t,a_t) - V_{\theta_V}(s_t)) \right ] \\
    %\mathcal{L}_Q(\theta_Q) & = \mathbb{E}_{(s_t,a_t,s_{t+1}) \sim \mathcal{D}} [ r(s_t,a_t) + \gamma \; V_{\theta_V}(s_{t+1})-Q_{\theta_Q}(s_t,a_t))^2 ]
%\end{align}
%with
an expectile loss \(L_2^\tau(u) = |\tau - \mathbbm{1}(u < 0)|u^2, \tau \in [0.5,1)\) on the difference between $V_{\theta_V}(s)$ and $Q_{\hat{\theta}_Q}(s,a)$ for any transition from the dataset. This   % the expectile loss, which corresponds to an asymmetric square loss which penalises positive values more than negative ones the more \(\tau\) tends to \(1\), consequently
leads  %the corresponding value function 
\(V_{\theta_V}(s_t)\) to lean towards \( \max_{\; a_{t+1} \in \mathcal{A}, \text{ st. } \pi_\beta(a_{t}|s_t) > 0} \; Q_{\hat{\theta}_Q}(s_t,a_t)\),  with \(\pi_\beta\) the  behavior policy of the training trajectories. The  policy is finally extracted using advantage weighted regression (AWR) from advantages estimated from \(V_{\theta_V}(s_t)\). 
%The use of two different networks is justified to train the value function only on the dataset action distribution without incorporating environment dynamics in the TD-error loss, which avoids the overestimation induced by lucky transitions. Then, the trained \(V_{{\theta}_V}(s_t)\) and \(Q_{{\theta}_{Q}}(s_t,a_t)\) are used to compute advantages to extract a policy \(\pi_{\theta_\pi}\) with advantage weighted regression (AWR):
%\begin{equation}
%\label{awr_loss}
%    \mathcal L_\pi(\theta_\pi) = -\mathbb E_{(s_t,a_t) \sim \mathcal D} \left[ \exp\left(\beta(Q_{\hat{\theta}_Q}(s_t,a_t) - V_{\theta_V}(s_t)\right)\log \pi_{\theta_\pi}(a_t|s_t) \right],
%\end{equation}
%with  \(\beta \in (0, +\infty]\) an inverse temperature. This correspond to the cloning of the demonstrations with a biais towards actions that present a higher Q-value.
\end{comment}

%\paragraph*{Hierarchical Implicit Q-Learning (HIQL)}
In the offline GCRL setting, the rewards are sparse, only giving signals for states where the goal is reached. Hence, as bad actions can be corrected by good actions and good actions can be polluted by bad actions in the future of the trajectory, offline RL methods are at risk of wrongly label bad actions as good one, and conversely good actions as bad ones. This leads to the learning of a noisy goal-condidtioned value function: \(\hat{V}(s_t,g) = V^*(s_t,g) + N(s_t,g)\) where \(V^*\) corresponds to the optimal value function and \(N\) corresponds to a noise. As the 'signal-to-noise' ratio worsens for longer term goals, offline RL methods such as IQL struggle when the scale of the GCRL problem increases, leading to noisy learning advantages %(as used in IQL's AWR weights  \cite{kostrikov2021offline} for instance)
, for which the noise overtakes the signal. To alleviate this issue, HIQL first proposes to learn a noisy goal conditioned action-free value function, inspired from IQL \cite{kostrikov2021offline}: 
\begin{equation}
    \label{iqlv}
    \mathcal{L}_V(\theta_V) = \mathbb{E}_{(s_t,s_{t+1},g) \sim \mathcal{D}} \left [ L_2^\tau(r(s_t,g) + \gamma V_{\hat{\theta}_V}(s_{t+1},g) - V_{\theta_V}(s_t,g)) \right ],
\end{equation}
using  
an expectile loss \(L_2^\tau(u) = |\tau - \mathbbm{1}(u < 0)|u^2, \tau \in [0.5,1)\) on the temporal difference of the value function, which %  between $V_{\theta_V}(s)$ and $Q_{\hat{\theta}_Q}(s,a)$ for any transition from the dataset. This   % the expectile loss, which corresponds to an asymmetric square loss which penalises positive values more than negative ones the more \(\tau\) tends to \(1\), consequently
%leads  %the corresponding value function 
%\(V_{\theta_V}(s_t)\) to lean towards \( \max_{\; a_{t+1} \in \mathcal{A}, \text{ st. } \pi_\beta(a_{t}|s_t) > 0} \; Q_{\hat{\theta}_Q}(s_t,a_t)\),  with \(\pi_\beta\) the  behavior policy of the training trajectories. 
aims at anticipating in-distribution sampling without querying the environment.  Then, it uses it to learn two policies \(\pi^h(s_{t+k}|s_t,g)\) to generate subgoals from the goal and \(\pi^l(a_t|s_t,g)\) to generate actions to reach the subgoals, in a hierarchical manner. This is done  with advantage weighted regression (AWR). %: 
\begin{comment}
\begin{align}
    \label{iql_losses}
    \mathcal{L}_{\pi^h}(\theta_h) & = \mathbb{E}_{(s_t,s_{t+k},g)}[\exp (\beta \cdot (V_{\theta_V}(s_{t+k},g) - V_{\theta_V}(s_t,g))) \log \pi_{\theta_h}^h(s_{t+k}|s_t,g)] \\
    \mathcal{L}_{\pi^l}(\theta_l) & = \mathbb{E}_{(s_t,a_t,s_{t+1},s_{t+k})}[\exp(\beta \cdot (V_{\theta_V}(s_{t+1},s_{t+k}) - V_{\theta_V}(s_t,s_{t+k})) \log \pi_{\theta_l}^l(a_t|s_t,s_{t+k})]
\end{align}
\end{comment}
With this division, each policy profits from higher signal-to-noise ratios, as the low-policy only queries the value function for nearby subgoals \(V(s_{t+1},s_{t+k})\) and the high policy queries the value function for more distant goal %diverse states leading to dissimilar values
\(V(s_{t+k},g)\).

\paragraph*{Quantizing Planner for Hierarchial Implicit Learning (QPHIL)} If HIQL shows significant improvements in offline GCRL problems compared to previous flat-policy methods, its performance depends on the right choice of the subgoal step \(k\). A high \(k\) would improve the high signal-to-noise ratio by quering more diverse subgoals but at the cost of decreasing the signal-to-noise ratio of the low policy. Conversly, a low \(k\) would improve the low signal-to-noise ratio by quering values for nearby goals but at the cost of the diversity of the high subgoals. Hence, HIQL might struggle for longer term goal reaching tasks as the low level performance imposes the choice of a sufficiently low \(k\), which lead to high frequency noisy high subgoal targets for the low policy to follow. QPHIL proposes to mitigate this issue by shifting the learning paradigm of the high policy into planning in a discretized learned space representation.
\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{.30\textwidth}
        \centering
        \includegraphics[height=.70\textwidth]{figures/qphil_1.png}
        \caption{Simpler high level planning}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.30\textwidth}
        \centering
        \includegraphics[height=.7\textwidth]{figures/qphil_2.png}
        \caption{Smoother low level targets}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.30\textwidth}
        \centering
        \includegraphics[height=.7\textwidth]{figures/qphil_3.png}
        \caption{Easier target conditioning}
    \end{subfigure}

    \caption{\textbf{Motivations behind QPHIL} (left) QPHIL aims to simplify the planning of the subgoals by leveraging the discrete tokens. (middle) Also, by doing so, QPHIL avoid the noisy high-frequency target subgoal updates by replanning only from token to token. (right) The subgoal reaching tasks are less demanding in conditioning for the low policy as it corresponds to the reaching of a entier subzone instread of a precise subgoal}
    \label{Motivations behind QPHIL}
\end{figure}





